Towards Safer Mobile Agents: Scalable Generation and Evaluation of Diverse Scenarios for VLMs

Vision Language Models (VLMs) are increasingly deployed in autonomous vehicles and mobile systems, making it crucial to evaluate their ability to support safer decision-making in complex environments. However, existing benchmarks inadequately cover diverse hazardous situations, especially anomalous scenarios with spatio-temporal dynamics. While image editing models are a promising means to synthesize such hazards, it remains challenging to generate well-formulated scenarios that include moving, intrusive, and distant objects frequently observed in the real world. To address this gap, we introduce \textbf{HazardForge}, a scalable pipeline that leverages image editing models to generate these scenarios with layout decision algorithms, and validation modules. Using HazardForge, we construct \textbf{MovSafeBench}, a multiple-choice question (MCQ) benchmark comprising 7,254 images and corresponding QA pairs across 13 object categories, covering both normal and anomalous objects. Experiments using MovSafeBench show that VLM performance degrades notably under conditions including anomalous objects, with the largest drop in scenarios requiring nuanced motion understanding.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_related-work.tex <==
\section{Related work}\label{sec:related}
% VLMの応用について
% 普通のVLM
%% VLMとは何か、なぜ説明するのか
%% VLMの構造について
%%% VLMはエンコーダー、でかLLM. projectorからなります
%%%% エンコーダ説明
%%%% でかLLM説明
%%%% projector説明
%%% 我々のベンチマークで測る能力について説明

%% VLMの応用
%%% robotとかMobile robotについて、普通のもの
%% 今までの研究の問題点
%%% これらのシナリオは主に一般的なシナリオで考えられており、anomalousなシナリオでのrobustnessについては明らかにしていない
%%% 実応用を考えるならばあまり起こり得ない状況についても状況理解する必要がある

% Safetyについて
%% これまでのVLM safetyのベンチマークについて、ここは具体例を挙げる
%%% 自動運転について
%%%% DriveBench, DriveQAなど、
%%% モバイルロボットについて
%%%% SA-Benchとかモバイルロボット

%% これまでの問題点
%%% あまりデータがないです。それはanomalousなシナリオやそもそも危険なシナリオがあまりないことに起因しています
%%

% 既存のデータセット, ベンチマークなど
%% 自動運転のデータセット
%%% 実画像のみのでかいデータセット
%%% シミュレーションのやつ

%% モバイルロボットのデータセット
%%% 実画像のやつ
%%% simulationのやつ

%%いいたいこと
%%% simulationのデータセットでは若干ドメインが違う
%%% 視覚的空間的なsafety
%%% 交通規則の理解
%%% 交通標識の認識
%%% 色々な天候でのロバストねす
%%% long-tailな状況への対応
%%%こららのデータセットは実画像を元にしているということが言いたい

%最後に、我々の研究では、commonなdangerous scnearioやanomalousな危険シナリオを構築します

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\input{tables/table_relatedwork}
%\subsection{Vision language models}
\subsection{Application of VLMs to mobility}
% general VLMs
VLMs~\cite{bai2025qwen25vltechnicalreport,NEURIPS2023_llava,wang2025internvl35advancingopensourcemultimodal,microsoft2025phi4minitechnicalreportcompact,steiner2024paligemma2familyversatile,openai2024gpt4ocard} have a remarkable ability to reason and understand across diverse environments.
%% VLMの応用
Ability of VLMs has been applied to mobility domains.
%%% robotとかMobile robotについて
An application for autonomous driving is a major application for VLMs~\cite{guo2025surds,sima2024drivelm,marcu2024lingoqavisualquestionanswering,tian2024drivevlmconvergenceautonomousdriving,xie2025DriveBenchvlmsreadyautonomousdriving,shi2025scvlmenhancingvisionlanguagemodel,li2025vladbenchfinegrainedevaluationlargevisionlanguage,wang2025metavqa}.
In the context of mobile robotics, VLMs are utilized for navigation tasks within social environments.~\cite{savlm_icra2025,payandeh2024socialllavaenhancingrobotnavigation,munje2025socialnavsubbenchmarkingvlmsscene}.
%% 今までの研究の問題点
%%% これらのシナリオは主に一般的なシナリオで考えられており、anomalousなシナリオでのrobustnessについては明らかにしていない
Despite these applications, previous research does not pay much attention to understanding of anomalous situation for VLMs.
%%% 実応用を考えるならばあまり起こり得ない状況についても状況理解する必要がある
Considering future application in the real world, measuring the ability of VLMs in not only frequently-happening scenarios but also anomalous scenarios is important.
%%% 我々の貢献
Our approach enables the generation for both common and anomalous scenarios with temporally dynamic and spatially diverse objects.


\subsection{Safety}
% Safety, こっちでは手法的な部分を扱うのが良い
The safety of VLMs in mobile agents, including autonomous vehicles and mobile robots, has become a significant topic of discussion recently.
%% Safetyについて
%%% 自動運転について
Autonomous driving for VLMs is frequently discussed from the perspective of safety.
SafeDriveRAG~\cite{ye2025safedriverag} improves the performance in safety-critical situations using RAG~\cite{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp}.
%%%% 実際の行動を問うやつとか
%%%% DriveBench, DriveQAなど、
%%% モバイルロボットについて
%%%% SA-Benchとかモバイルロボット
Safety of VLM-based mobile robots is also a critical topic. 
SA-VLMs~\cite{savlm_icra2025} addresses safe behavioral understandings of VLM-based dog mobile robots for visually impaired people.
Social-LLaVA~\cite{payandeh2024socialllavaenhancingrobotnavigation} tackles collision avoidance in the social situation for wheeled robots and legged robots with the VLM.
%%OODについて
%Safety in out-of-distribution (OOD) scenarios can cause critical result~\c.
%% これまでの問題点
%%% あまりデータがないです。それはanomalousなシナリオやそもそも危険なシナリオがあまりないことに起因しています
%%
The problem with these benchmarks for safety is the scarcity of long-tail anomalous data.
The reason for this scarcity is that there are few anomalous or inherently dangerous scenarios to begin with.
Using our method, we enable automatic generation of these dangerous scenarios.


\subsection{Benchmark and Datasets}
% 既存のデータセット, ベンチマークなど
Table~\ref{tbl:related} shows existing benchmarks for mobile robots and autonomous vehicles, and the position of our work.
%% 自動運転のデータセット
In autonomous driving, language-based datasets and benchmarks including open-ended VQA and MCQ have been proposed~\cite{marcu2024lingoqavisualquestionanswering,kim2018bddx,deruyttere-etal-2019-talk2car,sacheva2024rank2tell,Qian_2024_nusceneQA_AAAI,malla2023dramajointrisklocalization,wu2025nuPromptlanguage,tian2024drivevlmconvergenceautonomousdriving,guo2025surds}.
%%% 実画像のみのでかいデータセット
These datasets and benchmarks are constructed from established large datasets~\cite{sun2020WAYMOopenscalabilityperceptionautonomousdriving,Caesar_2020_CVPR_nuscenes,2023kitti,kim2018bddx} or originally collected data in the real world with language annotations.
%%% シミュレーションのやつ
Simulation-based methods, frequently employing CARLA~\cite{pmlr-v78-dosovitskiy17aCARLA}, are a feature of some works~\cite{wang2025metavqa,sima2024drivelm}.
These benchmarks handle diverse topics, including the ability of a steering decision considering spatial relation~\cite{sima2024drivelm}, robustness for weather conditions~\cite{xie2025DriveBenchvlmsreadyautonomousdriving}, and compliance of traffic regulations~\cite{wei2025driveqapassingdrivingknowledge,ye2025safedriverag,zhang2025SCDbenchevaluationsafetycognitioncapability}.
%%% 視覚的空間的なsafety
%The topic of steering decisions is often debated in the context of autonomous vehicles~\cite{}.
%%% 交通規則の理解
%One of the research areas of VLMs in autonomous driving focuses on adherence to traffic regulations~\cite{wei2025driveqapassingdrivingknowledge,ye2025safedriverag,zhang2025SCDbenchevaluationsafetycognitioncapability}.
%%% 色々な天候でのロバストねす
%The testing of VLMs for making decisions across varied weather conditions is also discussed~\cite{xie2025DriveBenchvlmsreadyautonomousdriving}.
%%% long-tailな状況への対応
%% モバイルロボットのデータセット
%%% 実画像のやつ
%%% simulationのやつ
%%% 視覚的空間的なsafety
In mobile robots, language-based datasets are also proposed~\cite{payandeh2024socialllavaenhancingrobotnavigation,savlm_icra2025,munje2025socialnavsubbenchmarkingvlmsscene}, which are also constructed from large datasets~\cite{karnan2022SCANDsociallycompliantnavigationdataset,park2020sideguide}.
The target of these benchmarks on mobile robots is to measure the ability of safer decision-making.
The problem with the existing benchmark is the lack of hazardous scenarios, including anomalous objects.
In our study, we focus on creating a benchmark for safer decision-making with our pipeline generating anomalous objects.


%%% simulationのデータセットでは若干ドメインが違うよね
%%%こららのデータセットは実画像を元にしているということが言いたい

%%%
%Benchmark for general safety of autonomous driving is created~\cite{zhang2025SCDbenchevaluationsafetycognitioncapability}.
%The other benchmark handles the abstract safety in open-end settings for autonomous agents in the simulation environment~\cite{lu2025isbenchevaluatinginteractivesafety,yin2025safeagentbenchbenchmarksafetask} and real-world environment~\cite{sermanet2025asimov1,Yue_2024_safevln}.
%While VLMs have been extensively evaluated across a range of tasks, including natural language understanding, scene interpretation, logical reasoning, code generation, and alignment with responsible AI principles such as the mitigation of biased, malicious, or harmful content. 

%However, their ability to comprehend and respond appropriately to physical safety concerns in grounded, real-world scenarios—particularly in domains like autonomous mobile agents in real-world situations remains less thoroughly explored. 
% As these models are increasingly deployed in environments where physical interaction and safety are critical, understanding their limitations and capabilities in such contexts is an important direction for future research.
% 我々が作るベンチマークではあるシチュエーションにおける次の移動アクションがsafeかどうかを問う包括的ベンチマークを作成する
%We tackle creating a benchmark for autonomous agents to decide where they move given the situational image, which harms.
\if0
▲XXX分野のサーベイ論文を複数挙げよ。 / Explain about multiple survey papers in the related area.


▲論文を複数挙げて、１個目の関連分野を説明せよ。 / Explain the first related subfield and several related papers.


▲論文を複数挙げて、N個目の関連分野を説明せよ。（この項目を個数分コピーしてください） / Explain the N-th related subfield and several related papers.


▲XXX分野の標準データセットについて説明せよ。 / Explain standard datasets in the related fields.


▲提案手法と類似手法A（＋類似手法B、類似手法C）との違いは何か？ / What is the difference(s) between the proposed and related methods?

\fi

\if0
%% VLMとは何か,なぜ説明するのか
%% VLMの構造について
Vision language models (VLMs) are mainly composed of three modules, including pretrained Large Language Model (LLM), a multimodal encoder, and a connector between an encoder and a LLM.
%%%% エンコーダ説明
For VLMs, pretrained Vision Transformer (ViT)~\cite{dosovitskiy2021vit} is widely used to extract a feature from an image.
%%%% projector説明
Extracted features are then input to a connector to align image features with text embeddings.
%%%% でかLLM説明
Finally, the aligned visual features are passed to a pretrained LLM, which handles reasoning and text generation. 
By leveraging its extensive linguistic knowledge, the LLM enables multimodal tasks such as image captioning, visual question answering (VQA), and instruction following. 
\fi

\if0
\subsection{Benchmark, Datasets}
% Autonomous driving 
In autonomous driving, several multimodal benchmarks~\cite{xie2025DriveBenchvlmsreadyautonomousdriving,marcu2024lingoqavisualquestionanswering,wang2025metavqa} are proposed based on the concept of driving with language.
% Mobile robots 
Open-end VQA Benchmarks to identify the capability of mobile robots are also proposed~\cite{savlm_icra2025,payandeh2024socialllavaenhancingrobotnavigation}. 
% Our method
DriveBench~\cite{xie2025DriveBenchvlmsreadyautonomousdriving} clarified that GPT-score is not a good metric since open-end VQA does not differ if no inputs are given to VLMs.
In the situation of autonomous mobile agents, the moving direction is constrained since moving directions are turning right, turning left, and going straight.
Our method focuses on multiple-choice question answering (MCQ).
The Comprehensive MCQ benchmark for autonomous agents, including autonomous vehicles and mobile robots, has not been proposed.
We tackle creating a comprehensive MCQ benchmark for autonomous mobile agents.
\fi


==> sec/3_HazardForge.tex <==
\section{HazardForge}
\label{sec:HazardForge}
%HazardForgeの概要
%% our approach why:HazardForgeを作ることになった課題を軽くさらい，だからHazardForgeを作りました
%% our approach how: HazardForgeをどのように作ったか軽く概要
% problem formulation
%% 今回扱う問題について概要
%% 一般的なMCQを次のように定義します．
%%%我々の問題こんな感じでMCQ定義します
%%%% image regionの導入,その理由について
%% 一般的な画像編集を次のように定義します
%%% 私たちの画像編集ではこんな感じです:マスクの話など
%% 望ましい出力について
%%% 多様性と唯一性、多様性が画像編集、唯一性がVLMのQuality assureに繋がる

% シナリオの分類
%% なぜこのシナリオを選ぶのか、なぜこのシナリオについて選んだのか、網羅性に対するWhyに答える
%%% distanceについてwhy,how
%%% motionについてwhy, how
%%% sudden intrusionについてwhy,how
%%% defaultについてwhy,how

% 生成の具体的な手法,
%% この章では何をやるか，なぜモジュールを作るのか
%% 図を用いて全体の説明を行う
%% 用語の定義
%%% 物体の概念の導入
%%%% その理由について
%%% 物体を示すテキストの導入
%%%% その理由について
%%% actionを示すテキストの導入
%%%% その理由について
%% 私たちこういうモジューるでいろんな生成パターン作りました
%% kontext方向づけ
%%% これを作った原因についておさらい
%%% アルゴリズムの説明
%%%% 正解の位置によって変えることを述べる 
%% paddingのやつ
%%% モジュールの概要目的
%%% ステップ1横を埋めます
%%% ステップ2その埋めたところに物体を生成します
%%% その画像の端を切り取ります
%% 消失点のやつ
%%% モジュールの概要目的モチベ
%%%% 遠くに生成するのはプロンプトだけでは難しい
%%%% なので我々は消失点を推定することでできる限り遠くにいるような物体を生成できるようにします
%%%モジュールの具体的説明
%% 唯一性保証
%%% モジュールの概要目的モチベ
%%% 具体的な手法
%%%% 方向と生成されているかどうか，
%%%%およびpaddingでは画像の中心にまたがっているかを確認した



%HazardForgeの概要
%% our approach why:HazardForgeを作ることになった課題を軽くさらい，だからHazardForgeを作りました
Among the safety benchmarks of VLMs, a lack of safety-critical situations is a challenge to address.
We propose HazardForge to mitigate the challenge.
%% our approach how: HazardForgeをどのように作ったか軽く概要
HazardForge utilizes image editing models to edit real-world images and VLMs to ensure the quality of images, respectively.

\subsection{Preliminary}
%% 今回扱う問題について概要
In this subsection, we address the formulation of multiple-choice questions and image editing, respectively.
% We also handles the desired output of image editing.

% 私たちMCQを次のように定義します．
\subsubsection{Direction-oriented question answering}
%\textcolor{red}{TODO: Write why we formulate the problem in this way. Why we focus on the direction of the action. }
In our study, we evaluate the capability of VLMs to identify the safe direction for mobile agents in an anomalous scene created by our pipeline. For ease of evaluation, we frame the task as direction-oriented question answering, where the model selects the safe driving direction (right, left, or straight) given an input image and question. Specifically, given an image ($I$) and a question ($q$), the model is asked to select the correct action $a$ from three options: $a_\text{R}$ (“steer right”), $a_\text{L}$ (“steer left”), and $a_\text{C}$ (“go straight”). We assume access to the dataset with this formulation and aim to create an anomalous scene based on the image and ground-truth safe direction. 

%At first, we define the multiple-choice question as follows. Denoting $\mathcal{I}$, $\mathcal{T}$ as a set of images and a set of texts, we formulate the multiple-choice question as $(I,q,a) \in \mathcal{I} \times \mathcal{T} \times \mathcal{T}$. 


%%%我々の問題こんな感じでMCQ定義します
%We denote the texts of actions indicating “steer to right,” “steer to left,” and “go straight” as $a_\text{R}$, $a_\text{L}$, $a_\text{C}$, respectively.
%Denoting $A = \{a_\text{R},a_\text{L},a_\text{C} \}$, our situation is formulated as $(I,q,a) \in \mathcal{I} \times \mathcal{T} \times A$.

We introduce notations to show the correspondence between an action of the ego and an image.
Assuming an image $I \in \mathbb{R}^{H \times W \times 3}$, we define an image region 
$\Omega(I) = \{(x,y) \mid 0 \le x < W,\; 0 \le y < H\}$ whose origin is at the bottom-left corner.
Fig.~\ref{fig:overview} shows that each action in $\{a_\text{L},a_\text{C},a_\text{R} \}$ corresponds to the destination defined as $
\Omega_\text{L}(I) = \{(x,y) \in \Omega(I) \mid 0 \leq x < \tfrac{W}{3}\}, 
\Omega_\text{C}(I) = \{(x,y) \in \Omega(I) \mid \tfrac{W}{3} \leq x < \tfrac{2W}{3}\}, 
\Omega_\text{R}(I) = \{(x,y) \in \Omega(I) \mid \tfrac{2W}{3} \leq x < W\}$, respectively.


\subsubsection{Image editing modules}
% 私たち画像編集を次のように定義します
We define the image editing inference in the following.
Let $M \in \{ \text{QIE}, \text{Kontext} \}$ be the pre-trained image editing model where QIE and Kontext denote Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport} and FLUX.1 Kontext~\cite{labs2025flux1kontextflowmatching}, respectively.
%% マスクの話
%Assuming an image $I \in \mathbb{R}^{H \times W \times 3}$, we define a image region $\Omega(I) = \{(x,y) \mid 0 \le x < W,\; 0 \le y < H\}$ whose origin is at the bottom-left corner.
Given a context image $I_{\text{in}} \in \mathcal{I}$ and a conditional mask $m \in \Omega(I_{\text{in}})$, and a prompt $t \in \mathcal{T}$, the output image $I_{\text{out}} \in \mathcal{I}$ is generated by sampling from the model as follows:
\begin{align*}
I_{\text{out}} \sim M(I_{\text{in}}, m, t)
\end{align*}


\if0
\subsubsection{Preliminaries for pipeline}
% 生成の具体的な手法
We introduce definitions of an object, movement direction, a prompt, and a specified mask as inputs for the image editing model.
%% 用語の定義
%%% 物体の概念の導入
%%%% その理由について
% We introduce a definition of an object to explain how our HazardForge enables generation of various objects including common and anomalous objects.
We denote a set of objects as $\mathcal{O}$ and an object as $o_k \in \mathcal{O}$ to be generated in each image region $\Omega_k(I)$ where $ k \in \{\text{L}, \text{C}, \text{R}\}$, respectively.
%%% 物体を示すテキストの導入
%%%% その理由について
We individually set a prompt $t_{o_k} \in \mathcal{T}$ of an object $o_k$, where $ k \in \{\text{L}, \text{C}, \text{R}\}$. % for each region $\Omega_k(I)$ as inputs for pretrained image editing model $M$.
%%% actionを示すテキストの導入
%%%% その理由について
We also introduce the classification of the movement direction.
Here, $\alpha_k \in E$ denotes the movement direction of the object $o_k$, where $E = \{ \text{LR}, \text{RL}, \text{F}, \text{B} \}$, which indicates moving left to right, right to left, forward, and backward, respectively.
We define a text prompt $t_{\alpha_k}$ indicating the moving direction $\alpha_k \in E$ as well.
%Then, we define the input of the algorithm detailed in Subsection~\ref{algo:hazardforge-return-I} as follows.
%%% mask regionの導入
%%%% その理由について
We denote $m_k \in \Omega(I)$ as the specified mask region where the model generate an object.
\fi




\if0
Shown in Fig.~\ref{fig:overview}, we construct Algorithm~\ref{algo:hazardforge-return-I}.
We denote inputs for our Algorithm~\ref{algo:hazardforge-return-I} as follows.
\begin{align*}
P = \{ (o_k,\alpha_k,m_k) \mid k \in \{\text{L}, \text{C}, \text{R}\} \}
\end{align*}
\textsc{GenAndCheck} in the Algorithm~\ref{algo:hazardforge-return-I} is selected from {$\textsc{GenAndCheck}_{\text{base}}$, $\textsc{GenAndCheck}_{\text{cut}}$, $\textsc{GenAndCheck}_{\text{dist}}$}, which we explain in the following.
\fi

\if0
\subsubsection{Requirements}
%% 望ましい出力について
%%% 多様性と唯一性、多様性が画像編集、唯一性がVLMのQuality assureに繋がる
There are two requirements for the desired benchmark in our setting.
The first desired requirement for outputs of images is a \textbf{diversity} of scenarios from general to anomaly for autonomous mobile agents.
The second desired requirement is \textbf{validity}, where the correct answer among the three options is uniquely determined by the outputs.
To meet two requirements, we propose modules, which we explain in the following.
\fi

\subsection{Pipeline}\label{subsec:scenario}

\if0
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{images/figure_method_all.pdf}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure*}
\fi

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/figure_method_overview.pdf}
    \caption{Example of correspondence between the answer of MCQ and image editing}
    \label{fig:overview}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{images/figure_method.pdf}
    \caption{Scenario wise generation method.}
    \label{fig:scenario_overview}
\end{figure*}

\subsubsection{Overview}
\if0
Aiming to test VLM's spatio-temporal understanding with various object, we designed eight patterns of image generation pipelines. 
It consists of a product of \{normal, anomalous\} objects $\times$ \{static, distance understanding, object's moving direction understanding, peripheral intrusion understanding  \} tests. Rendering anomalous objects in a scene covers long-tail dangerous situations, which is often the motivation of involving VLMs into decision making. The tests comprises one static scenario and three dynamic scenarios; which we design to evaluate  VLM's ability of understanding self-motion, understanding object motion, and early-stage danger perception.
\fi

%% saito's overview
% Given a triplet ((I, q, a)), our goal is to render anomalous objects in the image to simulate long-tail dangerous situations, while ensuring that the ground-truth action remains unchanged.  To comprehensively model such long-tail scenarios, we diversify (i) the object categories, and (ii) the spatial locations and the moving direction of the inserted objects within the scene while considering the consistency with the ground-truth action. 
% For the object categories, 

% パイプラインについて
In this subsection, we show the motivation of our generation pipeline and an overview of our pipeline shown in Fig.~\ref{fig:scenario_overview}.
%% motivation
%%% Intentionを先に書くとはどういうことなのだろう、howのもう一個上の層を書いてみるということか。いろんなシーンを生成するのがこのモジュールのintentionではないのか.いや描いてみるとわかったけどこれインテンションじゃない。モジュールのwhyが実装で置き換わった文章になっている
The reason why we create this pipeline is to render anomalous objects in a scene that covers long-tail dangerous situations, which is important to benchmark VLM's robustness.
The motivation of our pipeline is to generate various situations, which can evaluate VLM's ability of distance understanding, motion understanding, sudden intrusion understanding, and a default static scene understanding with common and anomalous objects.
%The motivation for using image editing models is to generate common and anomalous objects in these scenarios.
Distance understanding scenarios evaluate the ability of VLMs to
be aware that objects farther away generally pose less immediate risk than nearby ones.
Motion understanding scenarios investigate the capability of VLMs to decide a safe action, considering the movement direction of objects appearing in the scene.
Sudden intrusion scenarios probe about awareness of VLMs about unexpected appearances of objects from out of sight, a frequent occurrence in real-world scenarios. 
%VLMs must detect and reason about such events to ensure timely and safe decisions.
% We include a default static scene where all objects remain stationary and face the viewer. 
% This baseline scenario isolates complexity, allowing us to measure the fundamental decision-making ability of VLMs without confounding factors like motion or unpredictability.

%% 入力は何か
We input the original image $I_{\text{in}} \in \mathcal{I}$, a prompt $t_k \in \mathcal{T}$ of an object, and a conditional mask $m_k \subset \mathbb{R}^2$ to specify the location of generation, where each part $k \in \{\text{L}, \text{C}, \text{R}\}$ indicates the left, center and right section, respectively.
%% 出力は何か
The output is the image including added objects.
%% 中身の処理
HazardForge consists of the generation step and the quality checking step, where these steps are represented as a function $\textsc{GenAndCheck}$, detailed in the Appendix.
%%% Generation
%%%% motivation of gen
% The motivation of the generation step is rendering diverse objects in a scene that covers dangerous situations, which is often the motivation for involving VLMs in decision-making.
%%%% detail workflow
The objects are generated in the specified mask area with the specified movement direction using image editing models.
Shown in Fig.~\ref{fig:scenario_overview}, patterns of generation change according to each scenario.
We use motion image editing, intrusion image editing, and distance image editing for a motion understanding scenario, an intrusion understanding scenario, and a distance understanding scenario, which are explained in Subsection~\ref{subsec:motion}, \ref{subsec:intrusion}, \ref{subsec:distance}, respectively.
\if0
$\textsc{GenAndCheck}$ is selected from $\textsc{GenAndCheck}_{\text{base}}$, $\textsc{GenAndCheck}_{\text{intrusion}}$, $\textsc{GenAndCheck}_{\text{dist}}$ according to the scenario.
We use $\textsc{GenAndCheck}_{\text{base}}$ for a default static scene understanding and motion understanding.
We use $\textsc{GenAndCheck}_{\text{intrusion}}$, $\textsc{GenAndCheck}_{\text{dist}}$ for sudden intrusion understanding and distance understanding, respectively.
\fi
%%% Quality check
Then, the output of each image editing is input to the quality check module.
%%%% motivation of quality check
%The motivation of the quality check module is to check that the generation steps are aligned with the specified conditions, which helps to keep the quality of the benchmark.
%%%% detail workflow
The quality check module detailed in Subsection~\ref{subsec:vlmcheck} evaluates whether a generated object is completely generated in the specified area with the specified movement direction.
If quality checking fails, the generation is conducted iteratively.
If all of the quality checking goes well, the pipeline returns the output image.

% シナリオの分類



% We explain $\textsc{GenAndCheck}_{\text{cut}}$ and $\textsc{GenAndCheck}_{\text{dist}}$ in the following.
%We argue that our proposed evaluation patterns for mobility are comprehensive because they systematically cover three critical domains. These domains include the ability to understand the ego-vehicle's own motion (e.g., changes in perspective and distance); the ability to understand the motion of other agents (e.g., their direction and intent); and the ability to promptly detect objects (periphery), especially those appearing at the edges of the frame. We believe these three pillars effectively validate the core perceptual abilities required for safe navigation.




\subsubsection{Motion understanding}\label{subsec:motion}
%% kontext方向づけ
%%% motivation
The motivation of motion understanding scenario is to test VLMs' capacity to understand motion direction for the safe action.
Motion understanding ability is that
%The motivation of motion image editing is to generate a scenario testing 
%%% how
We describe how to generate scenarios for testing VLMs’ ability to understand motion direction.
% The detailed workflow of this scenario is in the Appendix.
We focus on the motion image editing approach shown in the top-right of Fig.~\ref{tbl:scenario-wise}.
%%% 役割
In this scenario, HazardForge generates the scene where the added object moves from the safe region selected from $\Omega_\text{L}(I_{\text{in}})$, $\Omega_\text{C}(I_{\text{in}})$, $\Omega_\text{R}(I_{\text{in}})$ specified by the answer $a$ of MCQ to the other adjacent region.
%where $k^* \in \{\text{L}, \text{C}, \text{R}\}$.
% The other object is generated by using default image editing, which is detailed in the Appendix.
%%% 入力
The inputs of motion image editing are the prompt $\text{Concat}(t_k,t')$ where a prompt $t'$  specifying the movement direction, a mask input $m_k = \Omega_k(I_{\text{in}})$, and an input image $I_{\text{in}}$.
%%% 出力
The output is the image where the oriented object is added.
%%% 流れ
Motion image editing outputs image $I_{\text{out}} \sim \text{Kontext}(I_{\text{in}}, m_k, \text{Concat}(t_k,t'))$
The detailed workflow of this scenario, other than motion image editing, is in the Appendix.
%%% アルゴリズムの流れ
%The movement direction is specified by the prompt $t_k$, and the movement direction of the generated object is validated by the quality check module.
%%%% 正解の位置によって変えることを述べる 
%We change the position and the movement direction of an object $o_k \in \mathcal{O}$ to be generated according to the answer $a$ of MCQ $(I,q,a) \in \mathcal{I} \times \mathcal{T} \times \mathcal{T}$. 
%In this scenario, we specify $m_k = \Omega_k(I_{\text{in}})$ as an input of the conditional mask for the image editing model.
% In this scenario, we introduce a generation pattern $P$ as an input for the algorithm.
%Denoting $k^* \in \{\text{L}, \text{C}, \text{R}\}$, the input $P$ for the algorithm is represented in the Appendix~\ref{appendix}.
% When $a_{k^*} = a_\text{C}$, the generative pattern is randomly selected.
%We apply the Algorithm~\ref{algo:genandcheck} $\textsc{GenAndCheck}_\text{base}$ for the Algorithm~\ref{algo:hazardforge-return-I} in this scenario.
%We use pretrained FLUX.1 Kontext~\cite{labs2025flux1kontextflowmatching} for the image editing model $M$.
% We detail the maximum number of trials $T_{\text{max}}$ by VLMCheck on Subsection~\ref{subsec:vlmcheck} in detail.



\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I_{\text{in}}$, \quad
       $P = \{(t_k, m_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ 
\State $I_{\text{cur}} \gets I_{\text{in}}$ 

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ 
    \For{$t = 1$ \textbf{to} $T_{\max}$}
        \State $(I_{\text{out}}, b_k) \gets \textsc{GenAndCheck}(I_{\text{cur}}, m_k, t_k)$
        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ 
            \State \textbf{break} 
        \EndIf
    \EndFor
\EndFor

\State $I \gets I_{\text{cur}}$ 
\State \Return $I$
\end{algorithmic}
\end{algorithm}

\if0
\begin{algorithm}
\caption{GenAndCheck Function}\label{algo:genandcheck}
\begin{algorithmic}[1]
\State \textbf{Input:} $I_{\text{cur}}$: current image, $m_k$: conditional mask, $t_k$: prompt
\Function{$\textsc{GenAndCheck}_{\rm base}$}{$I_{\text{cur}}, m_k, t_k$}
    \State $I_{\text{out}} \sim \text{Kontext}(I_{\text{cur}}, m_k, t_k)$
    \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}},m_k, t_k)$
    \State \Return $(I_{\text{out}}, b_k)$
\EndFunction
\end{algorithmic}
\end{algorithm}
\fi

%% 私たちこういうモジューるでいろんな生成パターン作りました
%% kontext方向づけ
%% paddingのやつ
\subsubsection{Sudden intrusion understanding}\label{subsec:intrusion}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{images/figure_method_padding.pdf}
    \caption{\textbf{The detailed workflow of our} intrusion image editing \textbf{.}}
    \label{fig:padding}
\end{figure}
%%% モジュールの概要目的
%%% motivation
The motivation of this scenario is to generate a scene where an object appears from outside of the sight to test the ability of VLMs to understand intrusion.
%%% how
Shown in the middle of Fig.~\ref{fig:scenario_overview}, we focus on the workflow of intrusion image editing, which generates an object appearing from outside of the sight.
We employ intrusion image editing since generating a partially visible object is difficult with only text prompts and masks in a traditional way.
%%% モジュールの入力
The input of intrusion image editing is a prompt $t_k \in \mathcal{T}$, an input image $I_{\text{in}}$, and the parameters $l,r \in \mathbb{R}$.
%%% モジュールの出力
Given in Fig.~\ref{fig:padding}, intrusion image editing outputs the image with the object partially visible at the edge.
%%% モジュールの流れ
Fig.~\ref{fig:padding} shows the workflow of intrusion image editing to generate objects that appear from the outside of the sight.
%We apply horizontal padding to the original input image $I_{\text{in}} \in \mathbb{R}^{H \times W \times 3}$.
%While padding is applied to the left side of the image for $k = \text{L}$, padding is applied to the right side for $k = \text{R}$.
%Denoting ${\rm Pad}_r^{\text{left}}(I_{\text{in}})$ and ${\rm Pad}_r^{\text{right}}(I_{\text{in}})$ as horizontal padding operations that add $r$ pixels to the left or right side of the image $I_{\text{in}}$, the padded image $I_{\text{in}}'$ is defined as:
\if0
\begin{align*}
I_{\text{in}}' =
\begin{cases}
{\rm Pad}_r^{\text{left}}(I_{\text{in}}),  & \text{if } k=\text{L} \\
{\rm Pad}_r^{\text{right}}(I_{\text{in}}), & \text{if } k=\text{R}
\end{cases} 
\end{align*}
\fi
% We outpaint the image $I_{\text{in}}' \sim \text{QIE}(I_{\text{in}}', \phi,  t)$ where a pre-defined prompt $t \in \mathcal{T}$ and an empty input $\phi$. 
%Shown in Step 1 in Fig.~\ref{fig:padding}, the outpainted image $I_{\text{in}}'$ is obtained by $I_{\text{in}}' \sim \text{QIE}(I_{\text{in}}', \phi,  t)$ where a padded image $I_\text{in}'$ an empty input $\phi$, a pre-defined prompt $t \in \mathcal{T}$. 
Shown in the step 1 in Fig.~\ref{fig:padding}, the $r \in \mathbb{R}$ pixel outpainted image $I_{\text{in}}' \in \mathbb{R}^{H \times (W + r) \times 3}$ is obtained by Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport} from the original input $I_{\text{in}} \in \mathbb{R}^{H \times W \times 3}$.
%Denoting the parameter $l \in \mathbb{R}$, 
The layout of the conditional mask is obtained as follows.
\begin{align*}
m_k^{\text{pad}} =
\begin{cases}
[r -l, r + l) \times [0, H), & \text{if } k = \text{L}, \\
[W - r - l, W - r + l) \times [0, H), & \text{if } k = \text{R},
\end{cases}   
\end{align*}
Given in the step 2 in Fig.~\ref{fig:padding}, we obtain the image $I_{\text{pad}} \sim \text{Kontext}(I_{\text{in}}', m_k^{\text{pad}}, t_k)$ including the added object in the image.
After eliminating specified $r$ pixels from $I_{\text{pad}}$ at the edge by cropping, we obtain the final result $I_{\text{out}}$.
We detail the generation workflow in the Appendix.
\if0
We denote the obtained procedure as 
\begin{align*}
    I_{\text{out}} \sim \text{\textsc{CutGen}}(I_\text{in},m_k, t_k)
\end{align*}
\fi
%In this scenario, we use the Algorithm~\ref{algo:genandcheck-cutgen} $\textsc{GenAndCheck}_{\rm cut}$ in the Algorithm~\ref{algo:hazardforge-return-I}.
% Then, we obtain the inputs of the Algorithm~\ref{algo:hazardforge-return-I} to generate scenarios of sudden intrusion understanding as follows.






%% 消失点のやつ
\subsubsection{Distance understanding}\label{subsec:distance}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{images/figure_method_vp.pdf}
    \caption{\textbf{The detailed workflow of our} \textsc{DistGen} \textbf{.}}
    \label{fig:vp}
\end{figure}
In this subsection, we focus on distance image editing shown in the bottom of Fig.~\ref{fig:scenario_overview}.
%%% Motivation
The motivation of this scenario is to generate a scene including an object in the distance to evaluate the ability of VLMs to consider the distance for safe decision-making.
We propose distance image editing since generating an object at a specified distance from the ego mobile agent is difficult with only text prompts with the traditional image editing model.
%To generate an object in the distance, we introduce vanishing point detection since the closer an object appears to the vanishing point on the image plane, the farther it is from the camera in reality, given a flat ground and a steady camera position in egocentric vision.
%%% 入力
The inputs of distance image editing are a vanishing point $p_{I_\text{in}} = (x',y') \in \Omega(I_\text{in})$, the parameter $d \in [0,1]$, an input image $I_{\text{in}}$,
%%% 出力
The output image is the image where the object is added in the distance shown at the bottom of Fig.\ref{fig:vp}.
%%%モジュールの流れ
Fig.~\ref{fig:vp} shows the overall workflow of our distance image editing.
Step 1 of the Fig.~\ref{fig:vp} shows the layout decision procedure.
%Here, we describe how to generate a mask region around the vanishing point.
We detect a vanishing point $p_{I_\text{in}} = (x',y') \in \Omega(I_\text{in})$ in an image $I_{\text{in}}$, using the rule-based method~\cite{luvpdetect2017}.
%Denoting the parameter $d \in [0,1]$, t
The layout of the conditional mask is decided as follows.
\begin{align*}
m_k^{\text{dist}} = \{ (x,y) \in \Omega_k(I_\text{in}) \mid |y - y'| \le d \cdot H \}.
\end{align*}
Given in the step 2 of Fig.~\ref{fig:vp}, we obtain the final sampling result $I_{\text{out}} \sim \text{Kontext}(I_{\text{in}}, m_k^{\text{dist}}, \text{Concat}(t_k,t_\text{dist}))$, where the pre-defined prompt $t_{\text{dist}}$ indicating the smaller object.
\if0
We represent this procedure as 
\begin{align*}
I_{\text{out}} \sim \textsc{DistGen}(I_{\text{in}}, m_k^{\text{dist}}, t_k))
\end{align*}
Using this notation, the input of the Algorithm~\ref{algo:genandcheck-distgen} is represented as follows.
\fi

Additionally, we create the default static scenario where objects do not have a moving direction.
The detail of the default static scenario is explained in the Appendix.
%We emark that the default static scenario uses an input for the Algorithm~\ref{algo:hazardforge-return-I} with the Algorithm~\ref{algo:genandcheck} $\textsc{GenAndCheck}_{\rm base}$ as follows.

% 唯一性

\subsubsection{Quality check}\label{subsec:vlmcheck}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{images/figure_method_check.pdf}
    \caption{The workflow of our quality check module}
    \label{fig:vlmcheck}
\end{figure}
%%% モジュールモチベ
The motivation of the quality check module is to ensure the validity of generated objects and their orientation.
%%% how
We employ a quality check module based on a VLM, which can verify whether the object is completely added and whether the object moves to the specified direction, respectively.
We employ Qwen3-VL-30B for our quality check module.
%入力について
The inputs of this module are an edited image $I_{\text{out}} \in \mathcal{I}$ of an image editing model, an input image $I_{\text{in}} \in \mathcal{I}$, the specified mask, the specified object, and the specified moving direction.
%出力について
The outputs of this module are the boolean value $b_k$, meaning completeness of the object and correctness of the moving direction.
% 流れについて
Fig.\ref{fig:vlmcheck} shows the overall workflow of the quality check.
For each output image $I_{\text{out}}$, we extract the region corresponding to the object mask $m_k$ and crop it from the image.
This cropped region is then input into the VLM and compare it with the corresponding region of $I_{\text{in}}$.
The VLM first verifies whether the object is visually present in the designated region. 
% It then checks whether the object's movement direction from $E$ corresponds to the specified action $\alpha_k \in E$.
It then checks whether the movement direction of the object corresponds to the specified moving direction.
% If all the things are verified, the function \textsc{VLMCheck} returns True. If else, it returns False.
The implementation and the validation quality of this module is detailed in the Appendix.


\if0
%----------------------------こっから下は60QAです

% ▲対象とするタスクの名称および内容は何か？ / What is the target problem?
%% 本研究で扱うタスクは画像編集です．
%% 画像編集とは入力画像と入力テキストに応じて画像を編集するタスクです


% ▲対象タスクの望ましい解・出力について説明せよ（何をもって良い解だとするのか）。 / What is the expected behavior of the system?
%% 望ましい出力としては，3つの選択肢のうち，正解が一意に定まるような状況を表現できている画像とします．目的はMCQに使用するための画像を生成することにあります．
%% 具体的には、望まれた方向に望まれた物体が生成されている状態を指します
%% 本研究のVLMのMCQでは，turn right, turn left, go straightの3つの選択肢から，安全な選択肢を選ぶという状況を想定しています．この手法では，3つの選択肢のうち，画像編集モデルにより3つのうちつだけが安全となるような画像が望ましい出力です．
%% そのため，ただひとつのみが安全な選択肢となっている状況を再現できている画像を生成することが望ましいansとなります．


%▲使用する用語を定義せよ。 / Define the terms used in the paper.
%% 本研究では、画像を見ている主体を移動体として扱い、それをAutonomous mobile agentsと呼ぶ
%% 本研究におけるsafetyとは移動エージェントが画像を与えられた時に，移動エージェントが行う行動によって接触などが起こり，主体もしくは接触された物体に被害が被る可能性がない場合をmobile safetyと定義する．
%% 本研究では動的な物体と静的な物体の生成を扱う．動的な物体をdynamic,静的な物体をstaticと定義する
%% 本研究では，生成される物体の方向を4つに分類します．forwardは主体に対して物体が向かってくる．left_to_rightは左から右へと移動している状態．right_to_leftは右から左へと移動している状態．backwardは主体から離れていくように動いていく状態です．
%% mobile safetyを達成するために，物体が生成される位置について定義する．(ここは数式でかく)



%% 我々のパイプラインでは4つの生成パターンを行います．Defaultは全ての物体が前を向いている状態を表します．Dynamicの場合は全ての物体がforwardの方向へと移動します．Moveは，物体の移動が行われる状態です．正解の位置に，ちょうど移動中の物体が生成され，他の位置に移動していきます．Farでは，正解の方向においては遠くに物体が配置されます．
%% これを数式で説明する



%▲対象タスクの代表例を示せ（図を付けること）。 / Explain a typical sample with a figure.
%% 後で
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{example-image-a}
    \caption{Example of our task}
    \label{fig:placeholder}
\end{figure}


%▲このタスクで与えられる入力は何か？ / What are the inputs of the task?
%% このタスクの入力では，現実世界の画像と，
%% turn right, turn left, go straightが選択肢として存在するMCQが与えられます。そのうち、正解は一つです
%% これらのactionは実際のデータセットから取り出されており，その方向に移動できることが保証されています．
The input for this task consists of a real-world image and the correct action among “turn right,” “turn left,” and “go straight.”
These actions are extracted from an actual dataset, and it is guaranteed that movement in the specified direction is possible.

%▲タスクで求められる出力は何か？ / What kind of outputs are expected for the task?
%% 出力としては，画像です
%% QAではturn right, turn left, go straightのうちひとつのみが安全な選択肢となっています
%% 
%Generated objects are classified to 4  defined as forward, backward,  





%▲本研究では何を扱わないか（＝何を前提にしているか）？ / What is the assumption in the paper?
%% 主体はある程度前方方向に速度がついた状態を仮定しており，stopなどの状況は扱わないものとします．
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I$, \quad
       $P = \{(o_k,\alpha_k,f_k,d_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ \Comment{Return the final, updated image}

\State $I_{\text{cur}} \gets I$ \Comment{Image used as the current input (initialized with the original image)}

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ \Comment{Initial validation result for this step}
    \For{$t = 1$ \textbf{to} $T_{\max}$}
        \If{$f_k = \text{cut}$}
            \State $I_{\text{out}} \gets \textsc{\textsc{CutGen}}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \ElsIf{$d_k < 1$}
            \State $I_{\text{out}} \gets \textsc{DistGen}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \Else
            \State $I_{\text{out}} \gets \textsc{EditModel}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \EndIf

        \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}}, o_k, \alpha_k,m_k)$

        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ \Comment{Update the input for the next $k$}
            \State \textbf{break} \Comment{Validation passed for this $k$; stop further trials}
        \EndIf
    \EndFor
    \Comment{Note: if all trials fail for this $k$, keep $I_{\text{cur}}$ unchanged}
\EndFor

\State $I \gets I_{\text{cur}}$ \Comment{Overwrite $I$ with the final updated image}
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi
%% 


% ▲本研究は何の手法を拡張した何を提案するものか？ / Which method do you extend?
%% この研究はAsimovで提案されたベンチマーク生成パイプラインを拡張したものになります。
%% 移動体における画像編集モデルを用いた安全性ベンチマークの生成パイプラインを提案しました.
%% 


% ▲提案手法で行った拡張は、上記の既存手法以外にも広く適用可能であることを説明せよ（＝他の既存手法に適用できないのであれば一般性がない拡張である）。 / Explain that the extensions made in the proposed method are widely applicable to other methods (i.e., if the extension cannot be applied to other methods, it would not be a generalized method).
%% 


% ▲提案手法と既存手法の違いを箇条書きせよ。 / List the differences between the proposed method and the conventional methods.
%% Why:AsimovベンチマークでのパイプラインではSemanctic Safetyと呼ばれる抽象的な安全性の概念を扱っていたのに対し，我々のベンチマークでは移動体の移動により引き起こされる事象に着目してベンチークを作成しました
%% How:Asimovベンチマークでは画像編集モデルを用いた危険な状況の生成を行っていましたが，それはVLMで画像を読み取り，そこから危険な状況を生み出すようなプロンプトを生成し，それをClosed modelのImagen 3に投げるというものでした．Asimovベンチマークで自動で作られたパイプラインでは生成された画像の品質保証を人間の手に頼っており，スケーラブルではありませんでした.我々の研究では，状況をより詳細に生成することが可能となっています．具体的には，生成される物体の種類や移動方向や生成される距離，画像からのはみ出しなどの多様な生成パターンを持っています．加えて，問題を分解してVLMによる品質保証を行い，所望の物体が生成されているかどうか，生成される物体の生成方向が正しいかなどのチェックを自動で行うことができ，スケーラブルです．

% ▲提案手法は何個の主要モジュールを有するか？各主要モジュールの名称を示せ。 / How many main modules does the proposed model have? Explain each method briefly.
%新規性を主張する部分には、査読者に注目してもらえる名前を付けるべし。
%% 主に2個です Cut moduleとfar moduleがあります




% ▲提案手法のモデル構造を示せ（図）。 / Explain the structure of the model.
%% あとで


% ▲入力を数式（またはx等の記号）で定義し説明せよ。各入力はそれぞれ何次元か？ / Define the input to the proposed method.
% 例えば、「モデルの入力はx_imgである。ここに、x_imgはmagnetogram画像を表す。」のように定義したとする。それにより、曖昧性を減少させると同時にスペースの無駄遣いを回避できる。
%% 



% ▲1個目のモジュールのmotivation・役割・入出力・構造を示して説明せよ。（この項目を個数分コピーしてください） / Explain the motivation, role, input-output, and structure of the N-th module. (Copy this question if needed)
%% Cut moduleは、主体の見える画面外から物体が飛び出してくる状況の画像を生成します。
%% motivation: 安全性における重要な考慮点の一つとして、視界の外側から物体が動いてくる場合などが挙げられます。画像の外側から物体が入ってくる状況をより忠実に生成するため、このmoduleを導入しました
%% 役割：，我々はcut moduleを作りました．これは$\Omega_\text{L}$もしくは$\Omega_\text{R}$に物体が生成される際に，それらの端で切り取られたような状況を生成するモジュールになります．
%% 入出力： 画像です
%% 

% ▲2個目のモジュールのmotivation・役割・入出力・構造を示して説明せよ。（この項目を個数分コピーしてください） / Explain the motivation, role, input-output, and structure of the N-th module. (Copy this question if needed)
%% motivation: 遠くにある物体は近くにある物体と比べ、安全性における考慮をする優先度が低いです。プロンプトのみで決まった位置により正確に生成するため、far moduleを作りました
%% 役割:far moduleは，物体を遠くにあるように生成するモジュールになります．
%% 構造消失点探索のアルゴリズムを利用します．消失点のうち，支配的な消失点を，最も多くの検出された線分を持つものとして扱います．消失点検出にはlu_vp_detectを用いました．消失点探索での検知する線分は60px以上にしてあります．

\if0
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I$, \quad
       $P = \{(o_k,\alpha_k,m_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ 
\State $I_{\text{cur}} \gets I$ 

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ 
    \For{$t = 1$ \textbf{to} $T_{\max}$}
            \State $I_{\text{out}} \sim \text{Kontext}(I_{\text{cur}}, m_k, t_k)$
        \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}}, t_k, c)$

        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ 
            \State \textbf{break} 
        \EndIf
    \EndFor
\EndFor



\State $I \gets I_{\text{cur}}$ 
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi

\if0
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I$, \quad
       $P = \{(o_k,\alpha_k,f_k,d_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ 
\State $I_{\text{cur}} \gets I$ 

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ 
    \For{$t = 1$ \textbf{to} $T_{\max}$}
        \If{$f_k = \text{cut}$}
            \State $I_{\text{out}} \gets \textsc{\textsc{CutGen}}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \ElsIf{$d_k < 1$}
            \State $I_{\text{out}} \gets \textsc{DistGen}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \Else
            \State $I_{\text{out}} \gets \textsc{EditModel}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \EndIf

        \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}}, o_k, \alpha_k,m_k)$

        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ 
            \State \textbf{break} 
        \EndIf
    \EndFor
\EndFor



\State $I \gets I_{\text{cur}}$ 
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_saito.tex <==
\section{HazardForge}
\label{sec:HazardForge}
We introduce HazardForge, a framework designed to automatically generate spatio-temporally diverse scenarios that include both common and anomalous objects, enabling evaluation of mobile agents' long-tail dangerous scenarios. 

Specifically, given a triplet of image, question, and ground-truth action indicating the direction of the safe direction for mobile agents, our goal is to render anomalous objects in the image to simulate long-tail dangerous situations, while ensuring that the ground-truth action remains unchanged.  
To comprehensively model such long-tail scenarios, we diversify (i) the object categories, and (ii) the spatial locations and the moving direction of the inserted objects within the scene while considering the consistency with the ground-truth action. 

In Sec.~\ref{sec:preliminary}, we describe the preliminary for our task definition, categories of rendered objects, and an image editing module. In Sec.~\ref{label:pipeline}, we describe the overall pipeline to render the objects considering the diversity of their spatial locations and the moving directions. 

\subsection{Preliminary}\label{sec:preliminary}

\noindent\textbf{Direction-oriented question answering.}
In our study, we evaluate the capability of VLMs to identify the safe direction for mobile agents in an anomalous scene created by our pipeline. 
For ease of evaluation, we frame the task as direction-oriented question answering, where the model selects the safe driving direction (right, left, or straight) given an input image and question. Specifically, given an image ($I$) and a question ($q$), the model is asked to select the correct action $a$ from three options: $a_\text{R}$ (“steer right”), $a_\text{L}$ (“steer left”), and $a_\text{C}$ (“go straight”). 
In the following, we denote the ground truth action as $a_{k^*}$ where $k^* \in \{\text{L},\text{C},\text{R} \}$.
We assume access to the dataset with this formulation and aim to create an anomalous scene based on the image and ground-truth safe direction. 

\noindent\textbf{Rendered categories.}
We aim to construct a benchmark that evaluates the performance of VLMs in recognizing both common and uncommon objects encountered by diverse mobile agents. Specifically, we select four common object categories—\textit{human, motorcycle, bicycle, and cone}—that frequently appear on roads, and nine anomalous object categories—\textit{rocks, debris, roadkill, dog, cat, deer, fox, pig, and raccoon}—that are rarely observed in standard mobile-agent datasets. 

%\subsubsection{Image editing}
\noindent\textbf{Image editing module.}
%We define the image editing inference in the following.
%Let $M \in \{ \text{QIE}, M \}$ be the pre-trained image editing model where QIE and Kontext denote Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport} and FLUX.1 Kontext~\cite{labs2025flux1kontextflowmatching}, respectively.
%% マスクの話
%Assuming an image $I \in \mathbb{R}^{H \times W \times 3}$, we define a image region $\Omega(I) = \{(x,y) \mid 0 \le x < W,\; 0 \le y < H\}$ whose origin is at the bottom-left corner.
Given an image $I_{\text{in}}$ and a conditional mask $m \in \Omega(I_{\text{in}})$, and a prompt $t \in \mathcal{T}$, the output image $I_{\text{out}} \in \mathcal{I}$ is generated by sampling from the model as follows:
\begin{align*}
I_{\text{out}} \sim M(I_{\text{in}}, m, t),
\end{align*}
where the text prompt specifies both the category and the direction of movement of the object to generate, and the mask specifies the location of the object. 
%The movement of direction is chosen from \textit{left}, \textit{right}, \textit{forward}, and \textit{backward}.


\noindent\textbf{Image regions to render objects.}
Given the three possible directions that the agent can choose, we horizontally split the image into three regions to clarify the location to render objects. Assuming an image $I \in \mathbb{R}^{H \times W \times 3}$, we define an image region $\Omega(I) = \{(x,y) \mid 0 \le x < W,\; 0 \le y < H\}$ whose origin is at the bottom-left corner.
Each action in $\{a_\text{L},a_\text{C},a_\text{R} \}$ corresponds to the destination defined as $
\Omega_\text{L}(I) = \{(x,y) \in \Omega(I) \mid 0 \leq x < \tfrac{W}{3}\}, 
\Omega_\text{C}(I) = \{(x,y) \in \Omega(I) \mid \tfrac{W}{3} \leq x < \tfrac{2W}{3}\}, 
\Omega_\text{R}(I) = \{(x,y) \in \Omega(I) \mid \tfrac{2W}{3} \leq x < W\}$, respectively. 
Depending on the ground-truth action and the variation of the spatial locations and moving directions of objects to insert, our pipeline chooses the split region as the target location for object rendering.

\subsection{Pipeline}\label{subsec:scenario}

%この図で伝えたいことは先に何か言語化する
%% HazardForgeには3つのシナリオがある
%% HazardForgeにはオブジェクトの種類を入れることができる
%% HazardForgeにはそれぞれのシナリオにおいてモジュールが存在し，場合によってはそのモジュールが利用される
%% HazardForgeには3つのシナリオがあり，
\if0
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/figure_method_overview.pdf}
    \caption{Example of correspondence between the answer of MCQ and image editing}
    \label{fig:overview}
\end{figure}
\fi

%この図で伝えたいことは先に何か書いておく＼
%% HazardForgeには3つのシナリオがある
%% HazardForgeにはそれぞれのシナリオにおいてモジュールが存在し，場合によってはそのモジュールが利用される
%% HazardForgeにはobjectがinputとして入ってくる, outputは
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/figure_method.pdf}
    \caption{Scenario wise generation method.}
    \label{fig:scenario_overview}
\end{figure}

\subsubsection{Overview}
\textcolor{red}{TODO: Rewrite overview fig. The fig has to describe we choose from three generation scenarios and categories.}
As shown in Fig.~\ref{fig:scenario_overview}, our pipeline diversifies the input image by the product of 13 categories and three generation scenarios consisting of \textit{motion scenario}, \textit{intrusion scenario}, and \textit{distance scenario} according to the ground truth of the question. 
% ここで力尽きた。11/13 00:30 by 齋藤
%The \textit{motion understanding} aims to check the ability of VLMs to capture the motion of 
%Fig.~\ref{fig:overview} 
% ここから先はtaniguchiが書く
We describe each scenario in the following.

\subsubsection{Motion scenario}\label{subsec:motion}
%% kontext方向づけ
%%% motivation
%%%% 特にこういうシナリオは大事.何か物体がある方向へと向かっている時は，それを迂回していくのが安全な判断である
%When an object is heading in a certain direction, maneuvering it is the safest decision considering the motion direction of the object, which is important for VLM's safety.
When an object moves in a certain direction, maneuvering around it is often the safest decision. 
Grasping how the object moves is essential for ensuring that the VLM can safely maneuver it.
%%%% 動く方向を予測して状況判断を下すのは重要な背景
%Deciding the safe action based on the expectation of the moving direction of an object in the scene mentioned above is an important ability for VLM's safety.
%%%% なのでMotion scenarioを作った
The motivation of the \textit{motion scenario} is to evaluate VLMs' ability to understand motion direction and make safe decisions to go around the object.
%%% how
%%%% howの概要
%In this situation, both the object and its path of movement pose dangers.
To simulate scenes for maneuvering, we consider scenarios where (i) the ground-truth action is restricted to either $a_\text{R}$ or $a_\text{L}$, and (ii) an object is positioned at the center region $\Omega_\text{C}(I_{\text{in}})$, moving toward the side opposite to the ground-truth region where $I_{\text{in}} \in \mathcal{I}$ is an input image.
The object's motion direction is set to \textit{go left} when the ground-truth action is $a_\text{R}$, and \textit{go right} when the ground-truth action is $a_\text{L}$ to make the ground-truth region appear safer than the opposite side of the ground-truth region.

To create the aforementioned object, we employ \textit{motion image editing}, which produces an object with the specified direction of movement.
%%%% どのような生成をするかの概要
% The detailed workflow of this scenario is in the Appendix.
% We focus on the \textit{motion image editing} approach shown in the top-right of Fig.~\ref{tbl:scenario-wise}.
%%% 役割
%In this scenario, HazardForge generates the scene where the added object moves from the safe region selected from $\Omega_\text{L}(I_{\text{in}})$, $\Omega_\text{C}(I_{\text{in}})$, $\Omega_\text{R}(I_{\text{in}})$ specified by the answer $a$ of MCQ to the other adjacent region.
%where $k^* \in \{\text{L}, \text{C}, \text{R}\}$.
% The other object is generated by using default image editing, which is detailed in the Appendix.
%%%% 流れ
%%%%% 入力
%\textit{motion image editing} generates an object at the center with a specified moving direction. 
\textit{motion image editing} creates an object positioned at the center with a designated direction of movement.
%We provide the prompt $\text{Concat}(t_\text{C}, t') \in \mathcal{T}$, where $t_\text{C} \in \mathcal{T}$ specifies the object type at the center, and $t' \in \mathcal{T}$ indicates the movement direction, chosen as either \textit{left to right} or \textit{right to left} based on the ground-truth action. 
We provide the prompt $t \in \mathcal{T}$, where specifies the object type at the center and the movement direction chosen to instruct as either \textit{go right} or \textit{go left} based on the ground-truth action. 
For \textit{motion image editing}, we adopt the mask $\Omega_\text{C}(I_{\text{in}})$ as input, because the object must be synthesized at the center of the image.
%The other input for \textit{motion image editing} is the image $I_{\text{in}}$ to be edited.
%%%%% 出力
Then, \textit{motion image editing} produces an output image $I_{\text{out}} \sim M(I_{\text{in}}, \Omega_\text{C}(I_{\text{in}}), t)$, where the object is generated at the center of the image and oriented according to the direction specified by $t$.
%%%%% チェック
Ensuring that the generated object conforms to the specifications given by $t$ is crucial for constructing the desired dataset. 
%The generated object in $I_{\text{out}} \in \mathcal{I}$ is evaluated for completeness and directional accuracy by the quality check module. 
% If the quality check fails, \textit{motion image editing} is repeated iteratively, as outlined in the Appendix.
%The detailed workflow of this scenario, other than \textit{motion image editing}, is in the Appendix.
%%% 出力
%The output is the image where the oriented object is added.
%%% アルゴリズムの流れ
%The movement direction is specified by the prompt $t_k$, and the movement direction of the generated object is validated by the quality check module.
%%%% 正解の位置によって変えることを述べる 
%We change the position and the movement direction of an object $o_k \in \mathcal{O}$ to be generated according to the answer $a$ of MCQ $(I,q,a) \in \mathcal{I} \times \mathcal{T} \times \mathcal{T}$. 
%In this scenario, we specify $m_k = \Omega_k(I_{\text{in}})$ as an input of the conditional mask for the image editing model.
% In this scenario, we introduce a generation pattern $P$ as an input for the algorithm.
%Denoting $k^* \in \{\text{L}, \text{C}, \text{R}\}$, the input $P$ for the algorithm is represented in the Appendix~\ref{appendix}.
% When $a_{k^*} = a_\text{C}$, the generative pattern is randomly selected.
%We apply the Algorithm~\ref{algo:genandcheck} $\textsc{GenAndCheck}_\text{base}$ for the Algorithm~\ref{algo:hazardforge-return-I} in this scenario.
%We use pretrained FLUX.1 Kontext~\cite{labs2025flux1kontextflowmatching} for the image editing model $M$.
% We detail the maximum number of trials $T_{\text{max}}$ by VLMCheck on Subsection~\ref{subsec:vlmcheck} in detail.


\if0
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I_{\text{in}}$, \quad
       $P = \{(t_k, m_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ 
\State $I_{\text{cur}} \gets I_{\text{in}}$ 

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ 
    \For{$t = 1$ \textbf{to} $T_{\max}$}
        \State $(I_{\text{out}}, b_k) \gets \textsc{GenAndCheck}(I_{\text{cur}}, m_k, t_k)$
        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ 
            \State \textbf{break} 
        \EndIf
    \EndFor
\EndFor

\State $I \gets I_{\text{cur}}$ 
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi

\if0
\begin{algorithm}
\caption{GenAndCheck Function}\label{algo:genandcheck}
\begin{algorithmic}[1]
\State \textbf{Input:} $I_{\text{cur}}$: current image, $m_k$: conditional mask, $t_k$: prompt
\Function{$\textsc{GenAndCheck}_{\rm base}$}{$I_{\text{cur}}, m_k, t_k$}
    \State $I_{\text{out}} \sim M(I_{\text{cur}}, m_k, t_k)$
    \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}},m_k, t_k)$
    \State \Return $(I_{\text{out}}, b_k)$
\EndFunction
\end{algorithmic}
\end{algorithm}
\fi


%% paddingのやつ
\subsubsection{Intrusion scenario}\label{subsec:intrusion}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/figure_method_padding.pdf}
    \caption{\textbf{The detailed workflow of our} \textit{intrusion image editing} \textbf{.}}
    \label{fig:padding}
\end{figure}
%%% モジュールの概要目的
%%%% なぜこんなことをするのか，それは切り取られた画像を作りたいから，なぜ切り取りたいのか
%%% motivation
%In a real-world scenario, the intrusion from out of the sight frequently happens, which is important for the safety of the VLM attached to the mobile agents.
%The motivation of this scenario is to generate these scenes to test the VLM's ability to understand intrusion.
In real-world environments, intrusions from outside the field of view occur frequently, posing significant safety concerns for VLMs integrated with mobile agents. 
The purpose of \textit{intrusion scenario} is to generate such scenes to evaluate the VLM's capability to comprehend intrusion events.
%%% how
%To generate these scenarios, we propose \textit{intrusion image editing}, which generates an object appearing from outside of the sight.
%%% シナリオの概要
%We describe the details of our generation methods in the following.In this scenario, the object is generated other than the safer region $\Omega_{k^*}(I)$ to make the safe option appear safer compared to other options.We configure the situation so that when $a_\text{R}$ or $a_\text{L}$ is the correct action, an object is generated at the center area corresponding to $a_\text{C}$ with the front view.At the edge of the area corresponding to $a_\text{R}$ or $a_\text{L}$, we have to generate the object with intrusion.
We outline the details of our generation methods as follows. 
Assuming an input image $I_\text{in} \in \mathcal{I}$, the object is placed other than the ground-truth region $\Omega_{k^*}(I_\text{in})$ to make the safe option appear comparatively safer than the alternatives. 
An object is generated in the central area $\Omega_{\text{C}}(I_\text{in})$ with a front-facing view, which is detailed in the Appendix. 
At the boundary of the region in $\Omega_{\text{R}}(I_\text{in})$ or $\Omega_{\text{L}}(I_\text{in})$, the object is generated to simulate an intrusion.
However, generating a partially visible object is difficult with only text prompts and masks in a traditional way.

%To generate these intrusive objects, we propose \textit{intrusion image editing}, which generates an object appearing from outside of the sight.
To create these intrusive objects, we introduce \textit{intrusion image editing}, which generates an object emerging from outside the field of view.
%%% difficulty
%We employ \textit{intrusion image editing} since generating a partially visible object is difficult with only text prompts and masks in a traditional way.
We utilize \textit{intrusion image editing} because generating a partially visible object using only text prompts and masks in the conventional approach is challenging.
%%% 流れ
%%%% モジュールの入力
%The input of \textit{intrusion image editing} is a prompt $t \in \mathcal{T}$ which specifies the object type and its direction, and an input image $I_{\text{in}}$.
%The input for \textit{intrusion image editing} consists of a prompt $t \in \mathcal{T}$ that specifies the object type and its orientation, along with an input image $I_{\text{in}}$. 
%and the parameters $l,r \in \mathbb{R}$.
%%%% モジュールの流れ
Fig.~\ref{fig:padding} shows the workflow of \textit{intrusion image editing} to generate objects that appear from the outside of the sight.
%We apply horizontal padding to the original input image $I_{\text{in}} \in \mathbb{R}^{H \times W \times 3}$.
%While padding is applied to the left side of the image for $k = \text{L}$, padding is applied to the right side for $k = \text{R}$.
%Denoting ${\rm Pad}_r^{\text{left}}(I_{\text{in}})$ and ${\rm Pad}_r^{\text{right}}(I_{\text{in}})$ as horizontal padding operations that add $r$ pixels to the left or right side of the image $I_{\text{in}}$, the padded image $I_{\text{in}}'$ is defined as:
% We outpaint the image $I_{\text{in}}' \sim \text{QIE}(I_{\text{in}}', \phi,  t)$ where a pre-defined prompt $t \in \mathcal{T}$ and an empty input $\phi$. 
%Shown in Step 1 in Fig.~\ref{fig:padding}, the outpainted image $I_{\text{in}}'$ is obtained by $I_{\text{in}}' \sim \text{QIE}(I_{\text{in}}', \phi,  t)$ where a padded image $I_\text{in}'$ an empty input $\phi$, a pre-defined prompt $t \in \mathcal{T}$. 
Step 1 in Fig.~\ref{fig:padding} illustrates the workflow of the layout decision used to create an object at the boundary of the image.
We convert the original image $I_{\text{in}} \in \mathbb{R}^{H \times W \times 3}$ into an $r \in \mathbb{R}$ pixel outpainted image $I_{\text{in}}' \in \mathbb{R}^{H \times (W + r) \times 3}$, enabling the subsequent natural insertion of the object into the image for Step 2.
%The $r \in \mathbb{R}$ pixel outpainted image $I_{\text{in}}' \in \mathbb{R}^{H \times (W + r) \times 3}$ is obtained by Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport} from the original input $I_{\text{in}} \in \mathbb{R}^{H \times W \times 3}$.
%Denoting the parameter $l \in \mathbb{R}$, 
Denoting the parameter $l \in \mathbb{R}$ to adjust the size of the mask, the configuration of the conditional mask to create the object positioned at the boundary of the scene is defined as follows.
\begin{align*}
m^{\text{pad}} =
\begin{cases}
[r -l, r + l) \times [0, H), & \text{if } a = a_\text{L}, \\
[W - r - l, W - r + l) \times [0, H), & \text{if } a = a_\text{R},
\end{cases}   
\end{align*}
Given a prompt $t \in \mathcal{T}$ specifying the object category and its orientation, we produce the object-integrated image $I_{\text{pad}} \sim M(I_{\text{in}}', m^{\text{pad}}, t)$ as illustrated in Step 2 of Fig.~\ref{fig:padding}. 
By cropping $I_{\text{pad}} \in \mathbb{R}^{H \times (W + r) \times 3}$ to remove $r$ pixels from the border, thereby forming a naturally intrusive object, we derive the final output image $I_{\text{out}} \in \mathbb{R}^{H \times W \times 3}$.
%%%% モジュールの出力
%Given in Fig.~\ref{fig:padding}, \textit{intrusion image editing} outputs the image with the object partially visible at the edge.
%%%% 他の場所の生成
%%%%% 正解の道が他の選択肢に比べて安全であるような状態にするため，$a_\text{R}$と $a_\text{L}$が正解の場合は中心に物体を生成するようにしました．詳細はappendixにあります
%We detail the generation workflow in the Appendix.
\if0
We denote the obtained procedure as 
\begin{align*}
    I_{\text{out}} \sim \text{\textsc{CutGen}}(I_\text{in},m_k, t_k)
\end{align*}
\fi
%In this scenario, we use the Algorithm~\ref{algo:genandcheck-cutgen} $\textsc{GenAndCheck}_{\rm cut}$ in the Algorithm~\ref{algo:hazardforge-return-I}.
% Then, we obtain the inputs of the Algorithm~\ref{algo:hazardforge-return-I} to generate scenarios of sudden intrusion understanding as follows.







%% 消失点のやつ
\subsubsection{Distance scenario}\label{subsec:distance}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{images/figure_method_vp.pdf}
    \caption{\textbf{The detailed workflow of our \textit{distance image editing}.}}
    \label{fig:vp}
\end{figure}
%In this subsection, we focus on \textit{distance image editing} shown in the bottom of Fig.~\ref{fig:scenario_overview}.
%%% Motivation
%%%% このシナリオの背景知識: 遠くにあるオブジェクトは近くにあるものよりSafeな行動の状況判断において重要でない．なぜなら移動体においては近くのものほど衝突などにつながりやすく危険な可能性が高いから
For mobile agents, nearby objects are more critical than distant ones, because a nearby object is more likely to cause a collision than a remote object.
%%%% このシナリオのVLMに対するモチベーション: そのような状況をVLMに理解させるのは重要である：why↑
The motivation of \textit{distance scenario} is to evaluate whether VLMs correctly interpret the nearby object as unsafe rather than focusing on the distant one.
\textit{distance scenario} includes a remote object and nearby objects.
%%%%シナリオについての概要，中身について
Assuming an input image $I_\text{in} \in \mathcal{I}$, we perform the image editing model to generate the nearby object with a front-facing view into all regions except the safe region $\Omega_{k^*}(I_\text{in})$, which is detailed in the Appendix.
A distant object is also generated at the safe region $\Omega_{k^*}(I_\text{in})$.
%%%% そのような状況を作るには難しさがある
However, generating an object appearing at a specified distance from the ego mobile agent is difficult with only text prompts for traditional image editing models.

%%%% だから\textit{distance image editing}を作った．
To overcome this challenge, we introduce \textit{distance image editing}, which creates an object that appears to be located far away within the scene.
%%%% \textit{distance image editing}とはどういうものか: \textit{distance image editing}では
%To create a distant object representation, we incorporate vanishing point detection. This is because, in egocentric vision, the nearer an object appears to the vanishing point on the image plane, the farther away it actually is from the camera, assuming a flat surface and a stable camera position.
%%% モジュールの流れ全体
Fig.~\ref{fig:vp} shows the overall workflow of our \textit{distance image editing}.
Step 1 of the Fig.~\ref{fig:vp} shows the layout decision procedure, which determines the area of the object to be generated in the safe region $\Omega_{k^*}(I_\text{in})$.
%%%% 入力
% The inputs of \textit{distance image editing} are a detected vanishing point $p_{I_\text{in}} = (x',y') \in \Omega(I_\text{in})$, the parameter $d \in [0,1]$, an input image $I_{\text{in}}$,
%Here, we describe how to generate a mask region around the vanishing point.
%%%% VPのglobalな理由
%%%% VP detectionのlocalな理由
Vanishing point (VP) detection is utilized to determine the layout of the conditional mask where the remote object is to be generated, since identifying the VP allows us to approximate where objects should be generated to appear further away.
In the input image $I_{\text{in}}$, the VP is represented as $p = (x',y') \in \Omega(I_\text{in})$ and is determined using the rule-based approach described in~\cite{luvpdetect2017}.
%%%% Conditional maskの導入，導入の理由
\textit{distance image editing} generates the remote object in $\Omega_{k^*}(I_\text{in})$.
%, where $\Omega_{k^*}(I_\text{in})$ indicates the safer direction for mobile agents to make the ground truth action $a_{k^*}$ appear safer than the other actions.
Denoting the parameter $d \in [0,1]$ to adjust the size of the mask, the layout of the conditional mask in the safer region $\Omega_{k^*}(I_\text{in})$ is determined as follows.
\begin{align*}
m_{k^*}^{\text{dist}} = \{ (x,y) \in \Omega_{k^*}(I_\text{in}) \mid |y - y'| \le d \cdot H \}.
\end{align*}
Given in Step 2 of Fig.~\ref{fig:vp}, we obtain the final sampling result $I_{\text{out}} \sim M(I_{\text{in}}, m_{k^*}^{\text{dist}}, \text{Concat}(t,t_\text{dist}))$, where the pre-defined prompt $t_{\text{dist}}$ indicates the smaller object such as \textit{make the object smaller} to make the object appear far away.


%%% シナリオに関する詳細
\if0
%%%% 出力
The output image is the image where the object is added in the distance shown at the bottom of Fig.\ref{fig:vp}.
\fi

%デフォルトシナリオについての説明
To compare the effect of each scenario, we additionally create the \textit{static scenario}, where the nearby objects with the front view are generated other than the safe region $\Omega_{k^*}(I_\text{in})$ corresponding to the correct action $a_{k^*}$.
%Additionally, we create the default static scenario where objects do not have a moving direction.
The detail of the \textit{static scenario} is explained in the Appendix.
%We emark that the default static scenario uses an input for the Algorithm~\ref{algo:hazardforge-return-I} with the Algorithm~\ref{algo:genandcheck} $\textsc{GenAndCheck}_{\rm base}$ as follows.

% 唯一性

\subsubsection{Quality check}\label{subsec:vlmcheck}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{images/figure_method_check.pdf}
    \caption{The workflow of our quality check module}
    \label{fig:vlmcheck}
\end{figure}
%%% モジュールモチベ
%%%% 各シナリオで意図したように生成が行われることが，良いデータセット作成には重要です
The successful creation of high-quality datasets hinges upon ensuring that the generation process in each scenario proceeds as intended. 
%%%% しかし画像編集モデルは時々，自分たちが意図した方向と違う方向を向いた生成を行ったり，そもそも生成を行ってくれない時があります．
However, image-editing models occasionally exhibit behavior that fails to produce any objects or deviates from the desired direction of generation.
%%%% 目的
The purpose of quality checking is to verify that the generated objects are complete and correctly oriented to filter out these unintended generations.

%%% how
% We employ a quality check module based on a VLM, which can verify whether the object is completely added and whether the object moves to the specified direction, respectively.
We employ a VLM-based quality check module that independently verifies (i) whether the object is fully inserted and (ii) whether it moves in the intended direction specified by the prompt $t \in \mathcal{T}$.
We utilize Qwen3-VL-30B for VLM of our quality check module.
% 流れについて
Fig.\ref{fig:vlmcheck} shows the overall workflow of the quality check module.
% Crop操作の理由．実際の操作
We execute cropping for each object mask to only compare the region where the object is generated.
For each output image $I_{\text{out}} \sim M(I_{\text{in}}', m, t)$ where the input image $I_{\text{in}} \in \mathcal{I}$, mask $m$, and a prompt $t \in \mathcal{T}$, we crop the region of $I_{\text{in}}$ and $I_{\text{out}}$ covered by the mask $m$.
We denote the cropped regions of $I_{\text{in}}$ and $I_{\text{out}}$ as $I_{\text{in}}'$ and $I_{\text{out}}'$, respectively.
%Cropped regions $I_{\text{in}}'$, $I_{\text{out}}'$, and the pre-defined prompts for verification are then input into the VLM.
%何をチェックするのか
The VLM first verifies whether the object is completely generated in the designated region specified by the mask $m$.
%We employ the prompt like \textit{Analyze the object's completeness in the edited image. Choose from: not generated, complete, incomplete} in this object's completeness verification procedure.
Cropped images $I_{\text{in}}'$, $I_{\text{out}}'$, and a prompt such as \textit{“Analyze the object's completeness in the edited image. Choose from: not generated, complete, incomplete”} are produced as inputs to the VLM.  
The result is accepted only if the VLM's output is \textit{complete}.  
In addition, the VLM checks the direction of the object's movement.
%実際のプロンプト
A cropped image $I_{\text{out}}'$ together with the pre-defined prompt \textit{“Analyze the object’s direction. Choose from: left, right, forward, backward”} are provided as inputs to the VLM.
The output only passes if the output of VLM matches the intended direction specified by the prompt $t$.
The implementation of this module and prompts are described in detail in the Appendix.
%入力について
%The inputs of the module are an edited image $I_{\text{out}} \in \mathcal{I}$ of an image editing model, an input image $I_{\text{in}} \in \mathcal{I}$, the specified mask, the specified object, and the specified moving direction.
%出力について
% The outputs of this module are the boolean value $b_k$, meaning completeness of the object and correctness of the moving direction.
% It then checks whether the object's movement direction from $E$ corresponds to the specified action $\alpha_k \in E$.
% It then checks whether the movement direction of the object corresponds to the specified moving direction.
% If all the things are verified, the function \textsc{VLMCheck} returns True. If else, it returns False.



\if0
%----------------------------こっから下は60QAです

% ▲対象とするタスクの名称および内容は何か？ / What is the target problem?
%% 本研究で扱うタスクは画像編集です．
%% 画像編集とは入力画像と入力テキストに応じて画像を編集するタスクです


% ▲対象タスクの望ましい解・出力について説明せよ（何をもって良い解だとするのか）。 / What is the expected behavior of the system?
%% 望ましい出力としては，3つの選択肢のうち，正解が一意に定まるような状況を表現できている画像とします．目的はMCQに使用するための画像を生成することにあります．
%% 具体的には、望まれた方向に望まれた物体が生成されている状態を指します
%% 本研究のVLMのMCQでは，turn right, turn left, go straightの3つの選択肢から，安全な選択肢を選ぶという状況を想定しています．この手法では，3つの選択肢のうち，画像編集モデルにより3つのうちつだけが安全となるような画像が望ましい出力です．
%% そのため，ただひとつのみが安全な選択肢となっている状況を再現できている画像を生成することが望ましいansとなります．


%▲使用する用語を定義せよ。 / Define the terms used in the paper.
%% 本研究では、画像を見ている主体を移動体として扱い、それをAutonomous mobile agentsと呼ぶ
%% 本研究におけるsafetyとは移動エージェントが画像を与えられた時に，移動エージェントが行う行動によって接触などが起こり，主体もしくは接触された物体に被害が被る可能性がない場合をmobile safetyと定義する．
%% 本研究では動的な物体と静的な物体の生成を扱う．動的な物体をdynamic,静的な物体をstaticと定義する
%% 本研究では，生成される物体の方向を4つに分類します．forwardは主体に対して物体が向かってくる．left_to_rightは左から右へと移動している状態．right_to_leftは右から左へと移動している状態．backwardは主体から離れていくように動いていく状態です．
%% mobile safetyを達成するために，物体が生成される位置について定義する．(ここは数式でかく)



%% 我々のパイプラインでは4つの生成パターンを行います．Defaultは全ての物体が前を向いている状態を表します．Dynamicの場合は全ての物体がforwardの方向へと移動します．Moveは，物体の移動が行われる状態です．正解の位置に，ちょうど移動中の物体が生成され，他の位置に移動していきます．Farでは，正解の方向においては遠くに物体が配置されます．
%% これを数式で説明する



%▲対象タスクの代表例を示せ（図を付けること）。 / Explain a typical sample with a figure.
%% 後で
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{example-image-a}
    \caption{Example of our task}
    \label{fig:placeholder}
\end{figure}


%▲このタスクで与えられる入力は何か？ / What are the inputs of the task?
%% このタスクの入力では，現実世界の画像と，
%% turn right, turn left, go straightが選択肢として存在するMCQが与えられます。そのうち、正解は一つです
%% これらのactionは実際のデータセットから取り出されており，その方向に移動できることが保証されています．
The input for this task consists of a real-world image and the correct action among “turn right,” “turn left,” and “go straight.”
These actions are extracted from an actual dataset, and it is guaranteed that movement in the specified direction is possible.

%▲タスクで求められる出力は何か？ / What kind of outputs are expected for the task?
%% 出力としては，画像です
%% QAではturn right, turn left, go straightのうちひとつのみが安全な選択肢となっています
%% 
%Generated objects are classified to 4  defined as forward, backward,  





%▲本研究では何を扱わないか（＝何を前提にしているか）？ / What is the assumption in the paper?
%% 主体はある程度前方方向に速度がついた状態を仮定しており，stopなどの状況は扱わないものとします．
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I$, \quad
       $P = \{(o_k,\alpha_k,f_k,d_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ \Comment{Return the final, updated image}

\State $I_{\text{cur}} \gets I$ \Comment{Image used as the current input (initialized with the original image)}

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ \Comment{Initial validation result for this step}
    \For{$t = 1$ \textbf{to} $T_{\max}$}
        \If{$f_k = \text{cut}$}
            \State $I_{\text{out}} \gets \textsc{\textsc{CutGen}}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \ElsIf{$d_k < 1$}
            \State $I_{\text{out}} \gets \textsc{DistGen}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \Else
            \State $I_{\text{out}} \gets \textsc{EditModel}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \EndIf

        \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}}, o_k, \alpha_k,m_k)$

        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ \Comment{Update the input for the next $k$}
            \State \textbf{break} \Comment{Validation passed for this $k$; stop further trials}
        \EndIf
    \EndFor
    \Comment{Note: if all trials fail for this $k$, keep $I_{\text{cur}}$ unchanged}
\EndFor

\State $I \gets I_{\text{cur}}$ \Comment{Overwrite $I$ with the final updated image}
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi
%% 


% ▲本研究は何の手法を拡張した何を提案するものか？ / Which method do you extend?
%% この研究はAsimovで提案されたベンチマーク生成パイプラインを拡張したものになります。
%% 移動体における画像編集モデルを用いた安全性ベンチマークの生成パイプラインを提案しました.
%% 


% ▲提案手法で行った拡張は、上記の既存手法以外にも広く適用可能であることを説明せよ（＝他の既存手法に適用できないのであれば一般性がない拡張である）。 / Explain that the extensions made in the proposed method are widely applicable to other methods (i.e., if the extension cannot be applied to other methods, it would not be a generalized method).
%% 


% ▲提案手法と既存手法の違いを箇条書きせよ。 / List the differences between the proposed method and the conventional methods.
%% Why:AsimovベンチマークでのパイプラインではSemanctic Safetyと呼ばれる抽象的な安全性の概念を扱っていたのに対し，我々のベンチマークでは移動体の移動により引き起こされる事象に着目してベンチークを作成しました
%% How:Asimovベンチマークでは画像編集モデルを用いた危険な状況の生成を行っていましたが，それはVLMで画像を読み取り，そこから危険な状況を生み出すようなプロンプトを生成し，それをClosed modelのImagen 3に投げるというものでした．Asimovベンチマークで自動で作られたパイプラインでは生成された画像の品質保証を人間の手に頼っており，スケーラブルではありませんでした.我々の研究では，状況をより詳細に生成することが可能となっています．具体的には，生成される物体の種類や移動方向や生成される距離，画像からのはみ出しなどの多様な生成パターンを持っています．加えて，問題を分解してVLMによる品質保証を行い，所望の物体が生成されているかどうか，生成される物体の生成方向が正しいかなどのチェックを自動で行うことができ，スケーラブルです．

% ▲提案手法は何個の主要モジュールを有するか？各主要モジュールの名称を示せ。 / How many main modules does the proposed model have? Explain each method briefly.
%新規性を主張する部分には、査読者に注目してもらえる名前を付けるべし。
%% 主に2個です Cut moduleとfar moduleがあります




% ▲提案手法のモデル構造を示せ（図）。 / Explain the structure of the model.
%% あとで


% ▲入力を数式（またはx等の記号）で定義し説明せよ。各入力はそれぞれ何次元か？ / Define the input to the proposed method.
% 例えば、「モデルの入力はx_imgである。ここに、x_imgはmagnetogram画像を表す。」のように定義したとする。それにより、曖昧性を減少させると同時にスペースの無駄遣いを回避できる。
%% 



% ▲1個目のモジュールのmotivation・役割・入出力・構造を示して説明せよ。（この項目を個数分コピーしてください） / Explain the motivation, role, input-output, and structure of the N-th module. (Copy this question if needed)
%% Cut moduleは、主体の見える画面外から物体が飛び出してくる状況の画像を生成します。
%% motivation: 安全性における重要な考慮点の一つとして、視界の外側から物体が動いてくる場合などが挙げられます。画像の外側から物体が入ってくる状況をより忠実に生成するため、このmoduleを導入しました
%% 役割：，我々はcut moduleを作りました．これは$\Omega_\text{L}$もしくは$\Omega_\text{R}$に物体が生成される際に，それらの端で切り取られたような状況を生成するモジュールになります．
%% 入出力： 画像です
%% 

% ▲2個目のモジュールのmotivation・役割・入出力・構造を示して説明せよ。（この項目を個数分コピーしてください） / Explain the motivation, role, input-output, and structure of the N-th module. (Copy this question if needed)
%% motivation: 遠くにある物体は近くにある物体と比べ、安全性における考慮をする優先度が低いです。プロンプトのみで決まった位置により正確に生成するため、far moduleを作りました
%% 役割:far moduleは，物体を遠くにあるように生成するモジュールになります．
%% 構造消失点探索のアルゴリズムを利用します．消失点のうち，支配的な消失点を，最も多くの検出された線分を持つものとして扱います．消失点検出にはlu_vp_detectを用いました．消失点探索での検知する線分は60px以上にしてあります．

\if0
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I$, \quad
       $P = \{(o_k,\alpha_k,m_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ 
\State $I_{\text{cur}} \gets I$ 

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ 
    \For{$t = 1$ \textbf{to} $T_{\max}$}
            \State $I_{\text{out}} \sim M(I_{\text{cur}}, m_k, t_k)$
        \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}}, t_k, c)$

        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ 
            \State \textbf{break} 
        \EndIf
    \EndFor
\EndFor



\State $I \gets I_{\text{cur}}$ 
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi

\if0
\begin{algorithm}
\caption{Generation and Validation Algorithm (return updated $I$)}\label{algo:hazardforge-return-I}
\begin{algorithmic}[1]
\State \textbf{Input} original image $I$, \quad
       $P = \{(o_k,\alpha_k,f_k,d_k) \mid k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}\}$, \quad
       max trials $T_{\max}$
\State \textbf{Output} $I$ 
\State $I_{\text{cur}} \gets I$ 

\For{$k \in \{\mathrm{L}, \mathrm{C}, \mathrm{R}\}$}
    \State $b_k \gets \text{False}$ 
    \For{$t = 1$ \textbf{to} $T_{\max}$}
        \If{$f_k = \text{cut}$}
            \State $I_{\text{out}} \gets \textsc{\textsc{CutGen}}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \ElsIf{$d_k < 1$}
            \State $I_{\text{out}} \gets \textsc{DistGen}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \Else
            \State $I_{\text{out}} \gets \textsc{EditModel}(I_{\text{cur}}, o_k, \alpha_k,m_k)$
        \EndIf

        \State $b_k \gets \textsc{VLMCheck}(I_{\text{cur}}, I_{\text{out}}, o_k, \alpha_k,m_k)$

        \If{$b_k = \text{True}$}
            \State $I_{\text{cur}} \gets I_{\text{out}}$ 
            \State \textbf{break} 
        \EndIf
    \EndFor
\EndFor



\State $I \gets I_{\text{cur}}$ 
\State \Return $I$
\end{algorithmic}
\end{algorithm}
\fi


==> sec/5_limitation.tex <==
\if0
\section{Limitation}~\label{sec:limitation}
% データセットの限界、画像編集モデルによって性能が変わるということ
Our approach, while effective in generating diverse hazardous scenarios, has several limitations including simplification of the problem formulation and simplified motion classification. 
First, the evaluation framework is simplified into an MCQ format, which does not fully capture the complexity of real-world decision-making for autonomous agents. 
Second, although dynamic scenarios are included, the representation of object motion is highly simplified and does not accurately reflect real-world diversities. 
Comprehensively covering dynamic scenarios remains for future work.
%Addressing these limitations will require extending the benchmark to incorporate richer interaction dynamics, more realistic motion modeling, and advanced generation techniques that better approximate real-world conditions.

%%%% Revision proposal (Hashimoto, just as a reference)
% Our approach, while effective in generating hazardous scenarios covering a comprehensive range of objects, has several limitations due to simplified problem modeling and limited patterns of generation pipelines. First, the evaluation framework is simplified into a MCQ format. This choice allows evaluating VLM's performance in safe decision-making but does not capture real-world complexity or allow reasoning validation. We believe that reasoning validation can be evaluated independently with VLM's safety. Second, although our pipeline includes self-motion, object motion, and peripheral intrusion, it does not cover diverse real-world dynamics. Comprehensively covering dynamic scenarios remains for future work.
\fi

==> tables/old_table.tex <==
\if0
\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{6pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{HazardForge creates more challenging benchmarks as seen in the performance drop by applying image editing.}\label{tbl:benchmark-wise}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcll}
\toprule 
Model          &     Source Data       & No edit & Edited      \\
\midrule 
 \multirow[c]{2}{*}{{{InternVL3.5}}}
   & DriveBench & 52.9    & 56.1\plusvalue{3.2}                        \\
               & SA-Bench   & 57.3    & 33.2\minusvalue{24.1}  \\ \arrayrulecolor{gray!40}\cline{1-4}\arrayrulecolor{gray}
\multirow[c]{2}{*}{$\text{LLAVA-NEXT}_\text{7B}$}
    & DriveBench & 54.3    & 50.2\minusvalue{4.1}    \\
               & SA-Bench   & 44.9    & 19.3\minusvalue{25.5}  \\ \arrayrulecolor{gray!40}\cline{1-4}\arrayrulecolor{black}
\multirow[c]{2}{*}{$\text{LLAVA-NEXT}_\text{13B}$}& DriveBench & 53.5    & 43.4\minusvalue{10.2}    \\
               & SA-Bench   & 77.3    & 53.6\minusvalue{23.7}   \\ \arrayrulecolor{gray!40}\cline{1-4}\arrayrulecolor{black}
\multirow[c]{2}{*}{Paligemma2}     & DriveBench & 38.2    & 34.0\minusvalue{4.3}     \\
               & SA-Bench   & 56.6    & 40.3\minusvalue{16.3}  \\ \arrayrulecolor{gray!40}\cline{1-4}\arrayrulecolor{black}
\multirow[c]{2}{*}{Phi4}           & DriveBench & 48.9    & 47.2\minusvalue{1.7}    \\
               & SA-Bench   & 75.7    & 70.9\minusvalue{4.8}   \\ \arrayrulecolor{gray!40}\cline{1-4}\arrayrulecolor{black}
\multirow[c]{2}{*}{$\text{Qwen2.5-VL}_\text{7B}$ }            
 & DriveBench & 54.6    & 36.5\minusvalue{18.1}    \\
               & SA-Bench   & 50.8    & 24.6\minusvalue{26.2}    \\ \arrayrulecolor{gray!40}\cline{1-4}\arrayrulecolor{black}
\multirow[c]{2}{*}{$\text{Qwen2.5-VL}_\text{32B}$ }& DriveBench & 52.0    & 45.8\minusvalue{6.2}    \\
               & SA-Bench   & 73.7    & 54.1\minusvalue{19.5}     \\
\bottomrule
\end{tabular}
}
\end{table}
\fi

\if0
\begin{table}[htbp]
\caption{Benchmark-wise}\label{tbl:benchmark-wise}
\begin{tabular}{cccccccc}
\toprule
Benchmarks   & InternVL3.5 & LLAVAN & LLAVAN13B & Pali2 & Phi4 & Q2.5-VL & Q2.5-VL-32B \\
\midrule
DriveBench         & 51.0        & 45.1       & 41.2           & 25.0       & 34.4 & 45.0       & 42.1           \\
SA-Bench          & 24.7        & 23.0       & 65.7           & 27.3       & 59.6 & 36.1       & 63.2  \\
\bottomrule
\end{tabular}
\end{table}
\fi

==> tables/table2_ver1.tex <==
\begin{table*}[tbp]
\centering
\setlength{\tabcolsep}{6pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{\textbf{Comparison of the performance among VLMs across different object categories.}}\label{tbl:category-wise}
\scalebox{0.9}{
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
category    & Size & bicycle & cat  & deer & dog  & fox  & human & rocks & debris & mcycle & pig  & raccoon & roadkill & cone & Total \\ \midrule
InternVL3.5 & 8B   & 47.8    & 40.0 & 39.0 & 46.2 & 40.2 & 50.8  & 55.9         & 53.7          & 44.2       & 43.9 & 43.2    & 55.8     & 55.9          & 46.5  \\
LLAVA-NEXT  & 7B   & 38.4    & 32.2 & 34.4 & 33.2 & 39.0 & 36.0  & 41.0         & 33.6          & 45.2       & 35.7 & 35.8    & 34.9     & 37.9          & 37.2  \\
LLAVA-NEXT  & 13B  & 57.5    & 33.8 & 42.2 & 45.5 & 40.2 & 44.1  & 53.4  & 57.8   & 56.9       & 46.2 & 42.8    & 46.5     & 48.1 & 47.7  \\
Paligemma2  & 10B  & 36.3    & 35.5 & 36.4 & 37.6 & 37.3 & 38.3  & 37.1         & 38.3          & 35.1       & 37.1 & 35.1    & 33.9     & 39.2          & 36.6  \\
Phi4        & 6B   & 66.5    & 45.3 & 48.3 & 54.9 & 44.4 & 58.7  & 60.2         & 65.9          & 63.6       & 55.8 & 55.8    & 62.8     & 60.3          & 57.2  \\
Qwen2.5-VL  & 7B   & 37.5    & 24.7 & 16.3 & 34.4 & 23.9 & 41.3  & 39.9         & 31.8          & 39.1       & 25.3 & 25.4    & 32.2     & 37.2          & 31.5  \\
Qwen2.5-VL  & 32B  & 54.1    & 40.4 & 34.0 & 51.9 & 39.2 & 58.7  & 53.0         & 46.5          & 54.0       & 44.0 & 52.6    & 51.5     & 54.2          & 49.3  \\
Average     &      & 48.3    & 36.0 & 35.8 & 43.4 & 37.7 & 46.8  & 48.6  & 46.8   & 48.3       & 41.1 & 41.5    & 45.4     & 47.5 & 43.7  \\ \bottomrule
\end{tabular}}
\end{table*}


==> tables/table2_ver2.tex <==
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{4pt}
\caption{Accuracy ($\uparrow$) of VLMs in the safe path MCQ task across object categories. Orange-colored cells are scores below the total score.}
\label{tbl:category-wise}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|c|cccc|ccccccccc|ccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multirow{2}{*}{Size} 
  & No
  & \multicolumn{4}{c|}{Normal objects} 
  & \multicolumn{9}{c|}{Anomalous objects} 
  & \multicolumn{3}{c}{Total} \\
& & edit & human & motorcycle & bicycle & cone & rocks & debris 
  & roadkill & dog & cat & deer & fox & pig & raccoon 
  & Norm. & Anom. & All \\
\midrule
InternVL3.5 & 8B
  & 54.8
  & 50.8           % human
  & \cellcolor{orange!20}44.2          % mcycle
  & 47.8           % bicycle
  & 55.9           % cone
  & 55.9           % rocks
  & 53.7           % debris
  & 55.8           % roadkill
  & \cellcolor{orange!20}46.2          % dog
  & \cellcolor{orange!20}40.0          % cat
  & \cellcolor{orange!20}39.0          % deer
  & \cellcolor{orange!20}40.2          % fox
  & \cellcolor{orange!20}43.9          % pig
  & \cellcolor{orange!20}43.2          % raccoon
  & 48.5           % Norm.
  & \cellcolor{orange!20}45.4          % Anor.
  & 46.5 \\         % All
LLAVA-NEXT & 7B
  & 50.3
  & \cellcolor{orange!20}36.0
  & 45.2
  & 38.4
  & 37.9
  & 41.0
  & \cellcolor{orange!20}33.6
  & \cellcolor{orange!20}34.9
  & \cellcolor{orange!20}33.2
  & \cellcolor{orange!20}32.2
  & \cellcolor{orange!20}34.4
  & 39.0
  & \cellcolor{orange!20}35.7
  & \cellcolor{orange!20}35.8
  & 40.7
  & \cellcolor{orange!20}35.5
  & 37.2 \\
LLAVA-NEXT & 13B
  & 63.5
  & \cellcolor{orange!20}44.1
  & 56.9
  & 57.5
  & 48.1
  & 53.4
  & 57.8
  & \cellcolor{orange!20}46.5
  & \cellcolor{orange!20}45.5
  & \cellcolor{orange!20}33.8
  & \cellcolor{orange!20}42.2
  & \cellcolor{orange!20}40.2
  & \cellcolor{orange!20}46.2
  & \cellcolor{orange!20}42.8
  & 52.8
  & \cellcolor{orange!20}45.1
  & 47.7 \\
PaliGemma2 & 10B
  & 46.0
  & 38.3
  & \cellcolor{orange!20}35.1
  & \cellcolor{orange!20}36.3
  & 39.2
  & 37.1
  & 38.3
  & \cellcolor{orange!20}33.9
  & 37.6
  & \cellcolor{orange!20}35.5
  & \cellcolor{orange!20}36.4
  & 37.3
  & 37.1
  & \cellcolor{orange!20}35.1
  & 36.8
  & \cellcolor{orange!20}36.6
  & 36.6\\
Phi4 & 6B
  & 60.2
  & 58.7
  & 63.6
  & 66.5
  & 60.3
  & 60.2
  & 65.9
  & 62.8
  & \cellcolor{orange!20}54.9
  & \cellcolor{orange!20}45.3
  & \cellcolor{orange!20}48.3
  & \cellcolor{orange!20}44.4
  & \cellcolor{orange!20}55.8
  & \cellcolor{orange!20}55.8
  & 62.6
  & \cellcolor{orange!20}54.5
  & 57.2\\
Qwen2.5-VL & 7B
  & 53.0
  & 41.3
  & 39.1
  & 37.5
  & 37.2
  & 39.9
  & 31.8
  & 32.2
  & 34.4
  & \cellcolor{orange!20}24.7
  & \cellcolor{orange!20}16.3
  & \cellcolor{orange!20}23.9
  & \cellcolor{orange!20}25.3
  & \cellcolor{orange!20}25.4
  & 38.8
  & \cellcolor{orange!20}27.9
  & 31.5\\
Qwen2.5-VL & 32B
  & 61.1
  & 58.7
  & 54.0
  & 54.1
  & 54.2
  & 53.0
  & \cellcolor{orange!20}46.5
  & 51.5
  & 51.9
  & \cellcolor{orange!20}40.4
  & \cellcolor{orange!20}34.0
  & \cellcolor{orange!20}39.2
  & \cellcolor{orange!20}44.0
  & 52.6
  & 54.9
  & \cellcolor{orange!20}46.5
  & 49.3\\
\midrule
Average & 
  & 55.6
  & 46.8
  & 48.3
  & 48.3
  & 47.5
  & 48.6
  & 46.8
  & 45.4
  & \cellcolor{orange!20}43.4
  & \cellcolor{orange!20}36.0
  & \cellcolor{orange!20}35.8
  & \cellcolor{orange!20}37.7
  & \cellcolor{orange!20}41.1
  & \cellcolor{orange!20}41.5
  & 47.9
  & \cellcolor{orange!20}41.6
  & 43.7\\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/table3_ver1.tex <==
\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{4pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{\textbf{Comparisons of degradation in MCQ accuracy after objects added in the scene by HazardForge}}\label{tbl:category-wise-difference}
\scalebox{0.95}{
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
% Please add the following required packages to your document preamble:
                               & bicycle                  & cat                      & deer                     & dog                      & fox                      & human                    & rocks                    & debris                   & motorcycle               & pig                      & raccoon                  & roadkill                 & cone                     \\ 
\midrule 
InternVL3.5                    & \cellcolor{red!40} -11.2 & \cellcolor{red!40} -11.5 & \cellcolor{red!40} -15.1 & \cellcolor{red!20} -7.0  & \cellcolor{red!20} -9.7  & \cellcolor{red!20} -3.0  & 2.9                      & \cellcolor{red!20} -3.7  & \cellcolor{red!40} -14.2 & \cellcolor{red!20} -8.5  & \cellcolor{red!40} -12.7 & 1.3                      & \cellcolor{red!20} -0.2  \\
$\text{LLAVA-NEXT}_\text{7B}$  & \cellcolor{red!40} -15.4 & \cellcolor{red!40} -17.2 & \cellcolor{red!40} -17.4 & \cellcolor{red!40} -16.5 & \cellcolor{red!40} -10.8 & \cellcolor{red!40} -13.4 & \cellcolor{red!20} -7.2  & \cellcolor{red!40} -18.7 & \cellcolor{red!20} -4.7  & \cellcolor{red!40} -13.6 & \cellcolor{red!40} -14.8 & \cellcolor{red!40} -16.6 & \cellcolor{red!40} -12.4 \\
$\text{LLAVA-NEXT}_\text{13B}$ & \cellcolor{red!40} -12.4 & \cellcolor{red!60} -26.1 & \cellcolor{red!60} -21.3 & \cellcolor{red!40} -16.2 & \cellcolor{red!60} -21.4 & \cellcolor{red!40} -17.4 & \cellcolor{red!20} -6.2  & \cellcolor{red!40} -12.2 & \cellcolor{red!20} -8.6  & \cellcolor{red!40} -15.9 & \cellcolor{red!60} -21.5 & \cellcolor{red!40} -16.3 & \cellcolor{red!40} -14.9 \\
Paligemma2                     & \cellcolor{red!40} -13.3 & \cellcolor{red!20} -3.8  & \cellcolor{red!20} -8.0  & \cellcolor{red!20} -7.8  & \cellcolor{red!20} -7.3  & \cellcolor{red!20} -7.3  & \cellcolor{red!20} -9.3  & \cellcolor{red!40} -11.3 & \cellcolor{red!40} -11.8 & \cellcolor{red!20} -8.4  & \cellcolor{red!40} -11.3 & \cellcolor{red!40} -10.6 & \cellcolor{red!20} -8.3  \\
Phi4                           & 2.1                      & \cellcolor{red!40} -11.7 & \cellcolor{red!40} -11.1 & \cellcolor{red!20} -4.4  & \cellcolor{red!40} -12.2 & 0.8                      & 3.5                      & \cellcolor{red!20} -0.5  & 0.5                      & \cellcolor{red!20} -2.2  & \cellcolor{red!20} -5.6  & 3.0                      & 0.0                      \\
$\text{Qwen2.5-VL}_\text{7B}$  & \cellcolor{red!40} -18.4 & \cellcolor{red!60} -27.6 & \cellcolor{red!60} -36.4 & \cellcolor{red!40} -17.5 & \cellcolor{red!60} -28.6 & \cellcolor{red!40} -12.9 & \cellcolor{red!40} -11.0 & \cellcolor{red!60} -23.3 & \cellcolor{red!40} -14.0 & \cellcolor{red!60} -26.6 & \cellcolor{red!60} -27.9 & \cellcolor{red!60} -22.9 & \cellcolor{red!40} -15.6 \\
$\text{Qwen2.5-VL}_\text{32B}$ & \cellcolor{red!40} -11.4 & \cellcolor{red!40} -17.2 & \cellcolor{red!60} -27.6 & \cellcolor{red!20} -8.2  & \cellcolor{red!40} -18.9 & \cellcolor{red!20} -1.8  & \cellcolor{red!20} -5.4  & \cellcolor{red!60} -21.0 & \cellcolor{red!20} -8.5  & \cellcolor{red!40} -15.1 & \cellcolor{red!20} -9.1  & \cellcolor{red!40} -10.3 & \cellcolor{red!20} -6.8 \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/table3_ver2.tex <==
\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{4pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{Degradation of safety MCQ accuracy by image editing. Cyan- and orange-colored cells are no degradation and more than 15 points degradation cases, respectively.}\label{tbl:category-wise-difference}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|rrrr|rrrrrrrrr|rrr@{}}
\toprule
\multirow{2}{*}{\multicolumn{1}{c}{Model}} & \multicolumn{4}{c|}{Normal objects} 
  & \multicolumn{9}{c|}{Anomalous objects} 
  & \multicolumn{3}{c}{Total} \\
  & human & motorcycle & bicycle & cone & rocks & debris & roadkill & dog & cat & dear & fox & pig & raccoon & Norm. & Anor.& All \\
\midrule
InternVL3.5
  & -3.0
  & -14.2
  & -11.2
  & -0.2
  & \cellcolor{cyan!15}2.9
  & -3.7
  & \cellcolor{cyan!15}1.3
  & -7.0
  & -11.5
  & \cellcolor{orange!15}{-15.1}
  & -9.7
  & -8.5
  & -12.7 
  & -9.2 & -7.8 & -8.3
  \\
$\text{LLAVA-NEXT}_{\text{7B}}$
  & -13.4
  & -4.7
  & \cellcolor{orange!15}{-15.4}
  & -12.4
  & -7.2
  & \cellcolor{orange!15}{-18.7}
  & \cellcolor{orange!15}{-16.6}
  & \cellcolor{orange!15}{-16.5}
  & \cellcolor{orange!15}{-17.2}
  & \cellcolor{orange!15}{-17.4}
  & -10.8
  & -13.6
  & -14.8 
  & -12.2 & -14.7 & -13.7\\
$\text{LLAVA-NEXT}_{\text{13B}}$
  & \cellcolor{orange!15}{-17.4}
  & -8.6
  & -12.4
  & -14.9
  & -6.2
  & -12.2
  & \cellcolor{orange!15}{-16.3}
  & \cellcolor{orange!15}{-16.2}
  & \cellcolor{orange!15}{-26.1}
  & \cellcolor{orange!15}{-21.3}
  & \cellcolor{orange!15}{-21.4}
  & \cellcolor{orange!15}{-15.9}
  & \cellcolor{orange!15}{-21.5} 
  & -12.1 & \cellcolor{orange!15}{-18.3} & \cellcolor{orange!15}{-16.0} \\
Paligemma2
  & -7.3
  & -11.8
  & -13.3
  & -8.3
  & -9.3
  & -11.3
  & -10.6
  & -7.8
  & -3.8
  & -8.0
  & -7.3
  & -8.4
  & -11.3
  & -11.8 & -8.5 & -9.7\\
Phi4
  & \cellcolor{cyan!15}0.8
  & \cellcolor{cyan!15}0.5
  & \cellcolor{cyan!15}2.1
  & 0.0
  & \cellcolor{cyan!15}3.5
  & -0.5
  & \cellcolor{cyan!15}3.0
  & -4.4
  & -11.7
  & -11.1
  & -12.2
  & -2.2
  & -5.6 
  & \cellcolor{cyan!15} 1.2 & -5.2 & -2.8 \\
$\text{Qwen2.5-VL}_{\text{7B}}$
  & -12.9
  & -14.0
  & \cellcolor{orange!15}{-18.4}
  & \cellcolor{orange!15}{-15.6}
  & -11.0
  & \cellcolor{orange!15}{-23.3}
  & \cellcolor{orange!15}{-22.9}
  & \cellcolor{orange!15}{-17.5}
  & \cellcolor{orange!15}{-27.6}
  & \cellcolor{orange!15}{-36.4}
  & \cellcolor{orange!15}{-28.6}
  & \cellcolor{orange!15}{-26.6}
  & \cellcolor{orange!15}{-27.9} 
  & \cellcolor{orange!15}{-16.7} & \cellcolor{orange!15}{-25.2} & \cellcolor{orange!15}{-21.9} \\
$\text{Qwen2.5-VL}_{\text{32B}}$
  & -1.8
  & -8.5
  & -11.4
  & -6.8
  & -5.4
  & \cellcolor{orange!15}{-21.0}
  & -10.3
  & -8.2
  & \cellcolor{orange!15}{-17.2}
  & \cellcolor{orange!15}{-27.6}
  & \cellcolor{orange!15}{-18.9}
  & \cellcolor{orange!15}{-15.1}
  & -9.1 
  & -9.6 & -14.6 & -12.7 \\
\midrule
Average
  & -7.9
  & -8.8
  & -11.4
  & -8.3
  & -4.7
  & -13.0
  & -10.3
  & -11.1
  & \cellcolor{orange!15}{-16.4}
  & \cellcolor{orange!15}{-19.6}
  & \cellcolor{orange!15}{-15.6}
  & -12.9
  & -14.7 
  & -10.1 & -13.5 & -12.2 \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/table4_ver1.tex <==
\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{4pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{Scenario-wise evaluation}\label{tbl:scenario-wise}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|c|ccc@{}}
\toprule
Models & Static & Motion & Intrusion & Distance \\
\midrule
InternVL3.5 & 52.8    & 35.7 & 50.8   & 42.6    \\
$\text{LLAVA-NEXT}_{\text{7B}}$  & 40.4    & 29.7 & 41.7   & 35.5    \\
$\text{LLAVA-NEXT}_{\text{13B}}$  & 45.1    & 50.5 & 42.2   & 39.7    \\
Paligemma2  & 37.2    & 38.6 & 34.3   & 35.4    \\
Phi4        & 63.9    & 51.7 & 57.7   & 49.1    \\
$\text{Qwen2.5-VL}_\text{7B}$  & 35.0    & 17.1 & 42.0   & 31.6    \\
$\text{Qwen2.5-VL}_\text{32B}$  & 54.4    & 31.8 & 65.9   & 40.4    \\
\midrule
Average     & 46.9    & 36.4 & 47.8   & 39.2   \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/table4_ver2.tex <==

\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{4pt}
\caption{Scenario-wise comparison. Cyan- and orange-colored cells are the easiest and hardest scenarios for each model.}\label{tbl:scenario-wise}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|c|c|ccc|c@{}}
\toprule
\multicolumn{1}{c|}{Models} & No edit & Static & Motion & Intrusion & Distance & Total\\
\midrule
InternVL3.5 &
  54.8 &
  \cellcolor{cyan!15}52.8 &
  \cellcolor{orange!15}35.7 &
  50.8 &
  42.6 &
  46.5\\
$\text{LLAVA-NEXT}_{\text{7B}}$  &
  50.3 &
  40.4 &
  \cellcolor{orange!15}29.7 &
  \cellcolor{cyan!15}41.7 &
  35.5 &
  37.2\\
$\text{LLAVA-NEXT}_{\text{13B}}$  &
  63.5 &
  45.1 &
  \cellcolor{cyan!15}50.5 &
  42.2 &
  \cellcolor{orange!15}39.7 &
  47.7\\
Paligemma2  &
  46.0 &
  37.2 &
  \cellcolor{cyan!15}38.6 &
  \cellcolor{orange!15}34.3 &
  35.4 &
  36.6 \\
Phi4        &
  60.2 &
  \cellcolor{cyan!15}63.9 &
  51.7 &
  57.7 &
  \cellcolor{orange!15}49.1 &
  57.2 \\
$\text{Qwen2.5-VL}_\text{7B}$  &
  53.0 &
  35.0 &
  \cellcolor{orange!15}17.1 &
  \cellcolor{cyan!15}42.0 &
  31.6 &
  31.5 \\
$\text{Qwen2.5-VL}_\text{32B}$  &
  61.1 &
  54.4 &
  \cellcolor{orange!15}31.8 &
  \cellcolor{cyan!15}65.9 &
  40.4 &
  49.3 \\
\midrule
Average     &
  55.6 &
  46.9 &
  \cellcolor{orange!15}36.4 &
  \cellcolor{cyan!15}47.8 &
  39.2 &
  43.7  \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/table_6and7_deleted.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htbp]
\small % 例: smallサイズに変更
\centering
\setlength{\tabcolsep}{4pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{Qwen2.5 VL-7B difference in DriveBench-based}\label{tbl:difference_analysis_robust-wise}
\scalebox{0.95}{
\begin{tabular}{@{}llllllllllllllll@{}}
\toprule
Category     & biterror                 & bright                   & camcrash                 & colorquant               & fog                      & framelost                & h256                     & lens                     & lowlight                 & motion                   & rain                     & saturate                 & snow                     & water                    & zoom                     \\ \midrule
bicycle      & \cellcolor{red!20} -6.4  & \cellcolor{red!20} -9.9  & \cellcolor{red!40} -14.7 & 0.0                      & \cellcolor{red!20} -2.6  & \cellcolor{red!20} -3.2  & 1.3                      & \cellcolor{red!20} -2.2  & 0.3                      & \cellcolor{red!20} -1.6  & \cellcolor{red!40} -17.3 & 1.0                      & 3.2                      & \cellcolor{red!20} -6.1  & \cellcolor{red!20} -0.3  \\
cat          & \cellcolor{red!40} -19.6 & \cellcolor{red!60} -23.9 & \cellcolor{red!60} -27.1 & \cellcolor{red!40} -16.1 & \cellcolor{red!60} -21.8 & \cellcolor{red!40} -13.6 & \cellcolor{red!40} -14.6 & \cellcolor{red!40} -19.3 & \cellcolor{red!40} -13.6 & \cellcolor{red!60} -21.1 & \cellcolor{red!60} -31.8 & \cellcolor{red!40} -13.6 & \cellcolor{red!40} -13.9 & \cellcolor{red!60} -22.5 & \cellcolor{red!40} -16.1 \\
deer         & \cellcolor{red!60} -31.2 & \cellcolor{red!60} -36.5 & \cellcolor{red!60} -37.4 & \cellcolor{red!60} -26.7 & \cellcolor{red!60} -30.3 & \cellcolor{red!60} -25.8 & \cellcolor{red!60} -25.6 & \cellcolor{red!60} -28.1 & \cellcolor{red!60} -24.2 & \cellcolor{red!60} -31.7 & \cellcolor{red!60} -42.4 & \cellcolor{red!60} -25.6 & \cellcolor{red!60} -25.6 & \cellcolor{red!60} -34.0 & \cellcolor{red!60} -26.4 \\
dog          & \cellcolor{red!20} -9.2  & \cellcolor{red!40} -14.8 & \cellcolor{red!40} -16.6 & \cellcolor{red!20} -6.2  & \cellcolor{red!40} -10.8 & \cellcolor{red!20} -8.4  & \cellcolor{red!20} -6.4  & \cellcolor{red!20} -8.2  & \cellcolor{red!20} -4.7  & \cellcolor{red!40} -10.7 & \cellcolor{red!60} -20.6 & \cellcolor{red!20} -4.7  & \cellcolor{red!20} -4.1  & \cellcolor{red!40} -12.5 & \cellcolor{red!20} -8.2  \\
fox          & \cellcolor{red!60} -20.0 & \cellcolor{red!60} -23.9 & \cellcolor{red!60} -26.0 & \cellcolor{red!40} -14.9 & \cellcolor{red!40} -18.8 & \cellcolor{red!40} -15.5 & \cellcolor{red!40} -15.8 & \cellcolor{red!40} -17.9 & \cellcolor{red!40} -12.5 & \cellcolor{red!60} -20.3 & \cellcolor{red!60} -30.8 & \cellcolor{red!40} -13.7 & \cellcolor{red!40} -13.1 & \cellcolor{red!60} -22.1 & \cellcolor{red!40} -12.8 \\
human        & \cellcolor{red!20} -3.1  & \cellcolor{red!20} -9.7  & \cellcolor{red!40} -10.0 & 1.0                      & \cellcolor{red!20} -2.4  & \cellcolor{red!20} -4.5  & 0.7                      & \cellcolor{red!20} -2.1  & 0.3                      & \cellcolor{red!20} -2.8  & \cellcolor{red!40} -14.8 & 5.5                      & 0.7                      & \cellcolor{red!20} -4.1  & \cellcolor{red!20} -0.3  \\
rocks  & \cellcolor{red!20} -8.5  & \cellcolor{red!40} -12.1 & \cellcolor{red!40} -14.3 & \cellcolor{red!20} -5.2  & \cellcolor{red!20} -8.1  & \cellcolor{red!20} -6.2  & \cellcolor{red!20} -5.2  & \cellcolor{red!20} -7.2  & \cellcolor{red!20} -2.3  & \cellcolor{red!20} -6.2  & \cellcolor{red!40} -16.3 & \cellcolor{red!20} -2.6  & \cellcolor{red!20} -0.3  & \cellcolor{red!40} -10.4 & \cellcolor{red!20} -6.5  \\
debris & \cellcolor{red!40} -14.9 & \cellcolor{red!60} -21.8 & \cellcolor{red!60} -25.3 & \cellcolor{red!40} -11.4 & \cellcolor{red!40} -14.4 & \cellcolor{red!40} -13.5 & \cellcolor{red!20} -9.2  & \cellcolor{red!40} -14.4 & \cellcolor{red!20} -8.3  & \cellcolor{red!40} -12.7 & \cellcolor{red!60} -26.6 & \cellcolor{red!20} -9.6  & \cellcolor{red!20} -5.2  & \cellcolor{red!40} -17.9 & \cellcolor{red!40} -13.1 \\
motorcycle   & \cellcolor{red!20} -0.6  & \cellcolor{red!20} -5.2  & \cellcolor{red!20} -8.4  & 6.3                      & 0.0                      & 2.6                      & 4.4                      & 3.7                      & 7.7                      & 2.8                      & \cellcolor{red!40} -10.9 & 7.3                      & 9.0                      & \cellcolor{red!20} -0.3  & 2.6                      \\
pig          & \cellcolor{red!60} -23.6 & \cellcolor{red!60} -27.2 & \cellcolor{red!60} -30.2 & \cellcolor{red!40} -18.6 & \cellcolor{red!60} -21.9 & \cellcolor{red!40} -17.5 & \cellcolor{red!40} -17.9 & \cellcolor{red!60} -20.0 & \cellcolor{red!40} -16.4 & \cellcolor{red!60} -21.1 & \cellcolor{red!60} -32.9 & \cellcolor{red!40} -16.9 & \cellcolor{red!40} -15.4 & \cellcolor{red!60} -23.2 & \cellcolor{red!40} -18.3 \\
raccoon      & \cellcolor{red!40} -19.9 & \cellcolor{red!60} -22.9 & \cellcolor{red!60} -26.5 & \cellcolor{red!40} -14.9 & \cellcolor{red!40} -18.5 & \cellcolor{red!40} -17.0 & \cellcolor{red!40} -14.2 & \cellcolor{red!40} -16.7 & \cellcolor{red!40} -12.4 & \cellcolor{red!40} -17.7 & \cellcolor{red!60} -30.7 & \cellcolor{red!40} -12.5 & \cellcolor{red!40} -11.5 & \cellcolor{red!60} -20.4 & \cellcolor{red!40} -15.2 \\
roadkill     & \cellcolor{red!40} -18.5 & \cellcolor{red!60} -27.0 & \cellcolor{red!60} -28.1 & \cellcolor{red!40} -14.0 & \cellcolor{red!40} -18.5 & \cellcolor{red!40} -19.7 & \cellcolor{red!40} -11.8 & \cellcolor{red!60} -21.4 & \cellcolor{red!40} -11.8 & \cellcolor{red!40} -19.1 & \cellcolor{red!60} -32.0 & \cellcolor{red!40} -14.0 & \cellcolor{red!40} -13.5 & \cellcolor{red!60} -20.8 & \cellcolor{red!40} -15.2 \\
cone & \cellcolor{red!20} -7.7  & \cellcolor{red!40} -10.0 & \cellcolor{red!40} -12.4 & \cellcolor{red!20} -1.2  & \cellcolor{red!20} -5.3  & \cellcolor{red!20} -3.5  & \cellcolor{red!20} -1.8  & \cellcolor{red!20} -4.4  & 1.8                      & \cellcolor{red!20} -5.3  & \cellcolor{red!40} -15.6 & 0.0                      & 1.8                      & \cellcolor{red!20} -7.1  & \cellcolor{red!20} -3.0  \\ \bottomrule
\end{tabular}}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htbp]
\setlength{\tabcolsep}{4pt} % 既定は6pt。2〜4ptまで詰めるのが無難
\caption{Scenario-wise comparison of the degradation after HazardForge}\label{tbl:scenario-wise_diff}
\begin{tabular}{@{}lllll@{}}
\toprule 
Top-level   Category & Static                   & Motion                   & Intrusion                & Distance  
\\
\midrule
InternVL3.5          & \cellcolor{red!20} -2.3  & \cellcolor{red!60} -25.4 & \cellcolor{red!20} -1.0  & \cellcolor{red!20} -4.7  \\
LLAVA-NEXT           & \cellcolor{red!20} -9.7  & \cellcolor{red!60} -23.8 & \cellcolor{red!20} -8.6  & \cellcolor{red!20} -9.7  \\
LLAVA-NEXT-13B       & \cellcolor{red!40} -10.7 & \cellcolor{red!60} -27.8 & \cellcolor{red!40} -14.3 & \cellcolor{red!40} -10.0 \\
Paligemma2           & \cellcolor{red!20} -9.0  & \cellcolor{red!40} -11.8 & \cellcolor{red!20} -9.1  & \cellcolor{red!20} -6.2  \\
Phi4                 & 3.0                        & \cellcolor{red!40} -16.3 & 1.0                        & \cellcolor{red!20} -0.7  \\
Qwen2.5-VL           & \cellcolor{red!40} -18.5 & \cellcolor{red!60} -38.7 & \cellcolor{red!40} -10.4 & \cellcolor{red!40} -16.1 \\
Qwen2.5-VL-32B       & \cellcolor{red!20} -7.5  & \cellcolor{red!60} -36.2 & 7.8                      & \cellcolor{red!40} -11.1 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_dataset_statistics.tex <==
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{4pt}

\caption{MovSafeBench statistics for each scenario and object category}
\label{tbl:dataset-statistics}
%\resizebox{\columnwidth}{!}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrrr|rrrrrrrrr|r}
\toprule
Scenario
 & Human & Motercycle & Bicycle & Cone & Rocks & Debris & Roadkill & Dog & Cat & Deer & Fox & Pig & Raccoon & Total\\
\midrule
Static & 144 & 331 & 27  & 350 & 348 & 301 & 258 & 289 & 102 & 168 & 123 & 303 & 349 & 3093\\
Motion & 162 & 298 & 165 &   - &   - &   - &   - & 300 & 208 & 257 & 234 & 273 & 297 & 2194\\
Intrusion  & 162 & 356 & 319 &   - &   - &   - &   - & 236 & 127 & 130 & 142 & 227 & 300 & 1999 \\
Distance  &  38 & 198 &  23 & 239 & 169 & 133 &  43 &  95 &  16 &  33 &  19 &  93 &  82 & 1181\\
\bottomrule
\end{tabular}
}
\end{table*}


